An Empirical Study of IoT Security Aspects at Sentence-Level in Developer Textual Discussions

IoT is a rapidly emerging paradigm that now encompasses almost every aspect of our modern life. As such, ensuring the security of IoT devices is crucial. IoT devices can differ from traditional computing, thereby the design and implementation of proper security measures can be challenging in IoT devices. We observed that IoT developers discuss their security-related challenges in developer forums like Stack Overflow(SO). However, we find that IoT security discussions can also be buried inside non-security discussions in SO. In this paper, we aim to understand the challenges IoT developers face while applying security practices and techniques to IoT devices. We have two goals: (1) Develop a model that can automatically find security-related IoT discussions in SO, and (2) Study the model output to learn about IoT developer security-related challenges. First, we download 53K posts from SO that contain discussions about IoT. Second, we manually labeled 5,919 sentences from 53K posts as 1 or 0. Third, we use this benchmark to investigate a suite of deep learning transformer models. The best performing model is called SecBot. Fourth, we apply SecBot on the entire posts and find around 30K security related sentences. Fifth, we apply topic modeling to the security-related sentences. Then we label and categorize the topics. Sixth, we analyze the evolution of the topics in SO. We found that (1) SecBot is based on the retraining of the deep learning model RoBERTa. SecBot offers the best F1-Score of 0.935, (2) there are six error categories in misclassified samples by SecBot. SecBot was mostly wrong when the keywords/contexts were ambiguous (e.g., gateway can be a security gateway or a simple gateway), (3) there are 9 security topics grouped into three categories: Software, Hardware, and Network, and (4) the highest number of topics belongs to software security, followed by network security.

==> background.tex <==
\section{Background}
In this section, we first offer a brief background overview of IoT domain (\sec\ref{sec:background-iot}). As noted in \sec\ref{sec:intro}, we studied four advanced language-based transformer models to detect IoT security related discussions in SO. We provide the background in the four models in \sec\ref{sec:background-info-transformer}.

\subsection{IoT}\label{sec:background-iot}
The internet of things (IoT) is a system of internet-connected objects (e.g., computing devices, digital machines) that can collect and transfer data over a wireless network without any human interactions~\cite{iot-intro,Atzori-SurveyIoT-ComputerNetwork2010,Gubbi-IoTVisionDirection-FGCS2013}. It can be things like a person with a heart monitoring implant, devices like a smart door that opens or closes automatically, or even microdevices like a biochip that can detect antibodies. 

% The idea of connected devices was first laid after the invention of the internet in the late 1960s \cite{iot-history}. For the first time, John Romkey connected a device to the internet with a TCP/IP protocol in 1990 \cite{iot-history-1990-madakam}\cite{iot-history-1990-Mattern}. After that, Kevin Aston first used the term IoT in his promotional speech on RFID back in 1999 \cite{iot-history-1999-Cisco}. Although IoT created some buzz and drew the attention of some executives, it did not get much attention until the 2010s. In 2011, market research company Gartner included an emerging technology `Internet of Things' \cite{iot-history-2011-wortmann}. Consequently, multiple companies around the globe started to work on `IoT'. And now IoT has surrounded us everywhere, from connected cars driving on the street, to home automation devices located in the house, smart office sensors embedded in the workplace, and fitness trackers worn on our bodies.

The exponential growth of IoT keeps the software industry busy developing new tools and technology and improving the existing system for a better user experience. By doing so, IoT developers are experiencing new challenges now and then. For example, security has become one of the main concerns in IoT devices as hackers can breach the device anytime to get confidential data. IoT security impacts the manufacturing of a device and measures necessary to protect IoT devices and networks. These days, IoT developers follow robust security portfolios to protect their devices from all types of vulnerabilities while developing the security level.
% For example, they follow cryptography \cite{iot-cryptography} tools to minimize communication attacks \cite{iot-communication-attack}, isolation measures to fend off software attacks \cite{isolation-attacking}, tamper mitigation to battle against physical attacks on the chip \cite{tamper-mitigation}, and so on.

\subsection{Transformer Models}\label{sec:background-info-transformer}
% In this paper, we have studied the accuracy of advanced language-based transformer models to detect IoT security-related discussions in SO. 
% The detection of security aspects in developer discussions was previously studied by Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019}, who investigated with 
% two shallow learning models (SVM and Logistic Regression). We are aware of no studies that focused on the development of 
% deep learning models to detect security aspect in developer discussions. 
In this paper, we have studied four advanced language-based transformer models to automatically detect security-related sentences in SO: BERT, RoBERTa, XLNet, and DistilBERT. In addition, we studied BERTOverflow, a BERT-based DL model that was pre-trained to learn SO-specific embedding~\cite{tabassum2020code}. Transformers \cite{transformers-kant} are attention based DL models that can handle sequential data like RNN (Recurrent Neural Network) \cite{rnn-model} and LSTM (Long Short Term Memory) \cite{lstm_recuurent_neural_net}. Unlike LSTM, the transformer models can process sequential data without any dependency between data sequence. This allows the models much more parallelism during the training and hence these models are faster than RNN, LSTM. Utilizing this feature, models are trained on large training dataset that was previously difficult using LSTM, RNN. These trained models are used for various language specific downstream tasks after fine-tuning the pre-trained models on the specific task-related domain (e.g., sentiment detection, machine translation).



% The models can be broadly divided into two types:
% \begin{enumerate}
%   \item Deep learning Models which are found to offer superior performance for text classifications (e.g., language translation) 
%   \item Transformer Models like the advanced pre-trained language models which are found to outperform other deep learning models for many text classifications (e.g., sentiment detection).
% \end{enumerate}
% \begin{table}[t]
%   \centering
%   \caption{Studied Deep Learning Models}
%     \begin{tabular}{lp{11cm}}\toprule
%     % {\textbf{Type}} &
%     \textbf{Name} & \multicolumn{1}{l}{\textbf{Rationale to Study}} \\
%     \midrule
%     % {RNN Models} & LSTM  & {Long Short Term Memory (LSTM) preserves history in sequences like word positions and occurrences, which is useful for text classification where context is important} \\
%     %       & Bi-LSTM & {Bidirectional LSTM analyzes an input two ways - from past to future and from future to past. 
%     %       This offers more contexts than LSTM (which is from past to future)} \\
%     % \midrule
%     % {Transformer Models} & 
%     BERT  &  BERT is designed to learn pre-trained contextual word representation by running of large volume of unlabeled texts. 
%     The transformer mechanism allows the encoder and decoder to see the entire input sequence at once.
%     \\
%         %  & 
%          XLNet &  XLNet offers better training methodology and uses more data for pre-training than BERT, which could increase its accuracy in learning.
%           \\
%         %   & 
%           RoBERTa & RoBERT uses more data and computation power to learn from the data. It also offers better training methodology than BERT and XLNet. As a result RoBERTa outperforms both BERT and XLNet on benchmark datasets (e.g., GLUE)
%           \\
%         %   & Albert &  Albert architecture offers a light-weight version of BERT architecture, without suffering much on the text classification performance. 
%         %   \\
%         %   & 
%           DistilBERT & DistilBERT is also a lightweight version of BERT in terms of the learned architecture and word embedding, while retaining more than 95\% of BERT performance.
%           \\
%           %& FunnelBERT &  \\
%           %& ELECTRA &  \\
%           BERTOverflow & BERTOverflow is an in-domain pretrained BERT. It is pretrained on SO dumps that include code snippets. As a result, it offers better performance on software domain-specific tasks.\\
%           \bottomrule
%     \end{tabular}%
%   \label{tab:studied-models}%
% \end{table}%

% \tbl\ref{tab:studied-models} overviews the studied models.  We offer architectural overview of the five models below. 
% \begin{figure}[!t]
%     \centering
%     \includegraphics[scale=.65]{images/BERT_Archi.pdf}
%     \caption{BERT Architecture Overview and Classification Processing}
%     \label{fig:BERT}
% \end{figure}

% RoBERTa, XLNet, DistilBERT and BERTOverflow all extend the base architecture of BERT. \fig\ref{fig:BERT} shows the internal
% architecture of Bidirectional Encoder Representations from Transformers (BERT)
% model. BERT takes embedded representation $(E_i)$ of words and does some multi-headed
% attention computation to create new intermediate representation $(Trm)$. Every
% layer compute multi-headed attention on the previous intermediate representation
% to create new one of identical size. The last intermediate layer of each word is
% fed to create final contextualized representation($T_i$) for each word. 

\bf{BERT} is trained on a large corpus like wikipedia, books, articles, and
etc in a self-supervised fashion to learn contextual word representation \cite{Delvin-BERTArch-Arxiv2018}. This
means it was pretrained on the raw texts only, with no humans labelling them. It
is an automatic process to generate inputs and labels from those texts. These
models were pretrained with two objectives- i) Masked Language
Modeling(MLM)\cite{salazar-etal-2020-masked} and ii) Next Sentence
Prediction(NSP)\cite{shi-demberg-2019-next-sentence-prediction}. BERT follow MLM
means model only predicts masked token instead of every next token. This is
because in multilayered model, lower layers leak information and allow a token
to itself in later layers. BERT model randomly masks 15\% of the words of a
sentence in the input then run the entire masked sentence through the model and
has to predict the masked words. It allows the model to learn a bidirectional
representation of the sentence. For NSP, model concatenates two masked sentences
as inputs during pretraining and then model predicts if the two sentences were
following each other or not. This way, model learns an inner representation of
the language that is used to extract features useful for downstream tasks.
Delvin at el.\cite{Delvin-BERTArch-Arxiv2018} provides two different
implementation of BERT- e.g., BERT-Base and BERT-Large.
% BERT-Base has a parameters
% of 110M with 12 layers, a hidden layer size of 768, and 12 self-attention heads.
% In comparison, BERT-Large has 340M parameters with 24 layers, a hidden layer
% size of 1,024, and 16 self-attention heads.



% Considering our dataset only
% consists of 6K samples which are not enough to tune 340M parameters, we choose
% BERT-Base model as suggested by Zhang at
% el.\cite{Zhang-SentimentDetectionSEBERT-ICSME2020}. \fig\ref{fig:BERT} (right) 
% shows how we used the BERT architecture for our security aspect detection.
% At first, a tokenizer takes the input sentences and represents the tokenized
% sentences. Then, this tokenized sentences are fed into BERT model. Finally, the
% embedded sentences are passed through the classifier to get final
% output (security or non-security).




%\gias{draw an explain a BERT architecture similar to \url{https://www.analyticsvidhya.com/blog/2019/09/demystifying-bert-groundbreaking-nlp-framework/}}
%\gias{use the above architecture to explain how BERT differs from LSTM and Bi-LSTM}

\bf{XLNet} is pre-trained using an autoregressive method to learn bidirectional contexts by maximizing the expected likelihood over all permutations of the input sequence factorization order \cite{Yang-Xlnet-Arxiv2020}. Like BERT, this model also use the BooksCorpus and English Wikipedia as part of pretraining
data. In addition, Giga5, ClueWeb 2012-B, and Common Crawl data were used for pretraining. Yang at el.\cite{Yang-Xlnet-Arxiv2020} proposed this model showing under comparable experiment settings, XLNet outperforms BERT on 20 tasks, often by a large margin, including question answering, natural language inference, sentiment analysis, and document ranking.

\bf{RoBERTa} is the most used and optimized BERT model for classification task \cite{Liu-Roberta-Arxiv2019}. Roberta model is pretrained on BookCorpus, a dataset consisting of 11,038 unpublished books, English Wikipedia (excluding lists, tables and headers), CC-News: a dataset containing 63 millions English news articles, OpenWebText: an opensource recreation of the WebText,
Stories: a dataset containing a subset of CommonCrawl data. Contrary to BERT, the masking is done dynamically during pretraining (e.g., it changes at each epoch and is not fixed) \cite{Liu-Roberta-Arxiv2019}.
% Most used RoBERTa model is Roberta-Base. It has 125M parameters with 12 layers, 768 neurons per layer and 12 self-attention heads. 

\bf{DistilBERT} is smaller and faster than BERT, which was pretrained on the same corpus, using the BERT base model as a teacher \cite{Distil-Bert}. This model has a triple loss combining language modeling, distillation and cosine-distance losses that makes the model smaller in parameter size while preserved in performance. The DistilBERT model has 40\% lesser number of parameters than its base model BERT. 

% Following Pipalia at el.\cite{Distil-Bert} and Adoma at el.\cite{Adoma-Distil-Bert}, we use DistilBERT-Base model for our classification task.

\bf{BERTOverflow} has the same architecture as BERT. This model has purposefully been created for software domain-specific tasks like sequence classification, entity model named entity recognition, etc. Instead of training on generic English literature like Wikipedia or BooksCorpus, the model is trained on SO dumps- i.e., posts, comments, and answers. Thus, the model learns to represent software-specific contexts. This model has shown better performance than BERT in some SO-specific tasks.


==> data.tex <==
\section{A Benechmark of IoT Security Aspects}\label{sec:studied-datasets}
% We studied two datasets: The API review dataset used in Opiner tool by Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019} and 
% a new dataset with 53K IoT posts from Stack Overflow. We discuss the datasets below.
% \subsection{Opiner API Review Dataset} \label{sec:opiner-data-setup}
% We use the Opiner benchmark dataset~\cite{Uddin-OpinionValue-TSE2019}, which 
% was created from 1,338 SO posts. The dataset contains 4,522 sentences, each labeled with 11 API aspects like security, performance, etc. 
% The security related sentences were mainly collected from questions tagged as `authentication' and `cryptography'. 
% For our experiment, we used only security aspect. Hence, we labeled each sentence in the benchmark as 1 (i.e., security-related) or 0  (otherwise). 
% We find 225 duplicate sentences in the Opiner benchmark, i.e., sentences from a given SO thread were mistakenly added twice in the original dataset. 
% We removed those before our experiment, which resulted in total 4,297 distinct sentences in the benchmark. 
% The final benchmark is imbalanced; it has 163 sentences labeled as 1 and 4,134 labeled as 0 (ratio = 4\%). 
% % \begin{table*}[h]
% %   \centering
% %   \caption{Opiner Dataset Details}
% %     \begin{tabular}{ccc} \toprule
% %     \textbf{\#Security} & \textbf{\#Non-Security} & \textbf{\#Total} \\ 
% %     \midrule
% %     163 & 4134 & 4297\\
% %     \bottomrule
% %     \end{tabular}%
% %   \label{tab:opiner-details}%
% % \end{table*}%
% 
\subsection{IoT Data Collection}\label{sec:iot-data-collection}
We follow three steps to collect SO posts related to IoT discussions: \begin{inparaenum}[(1)]
\item Download SO dataset,
\item Identify IoT tagset in the dataset, and
\item Download IoT posts from the dataset based on the IoT tagset.
\end{inparaenum} We describe the steps below.

\nd\bf{\ul{Step 1. Download SO Dataset.}} 
%To determine the IoT topics in SO, we first need a list of all questions and answers in SO. 
%We picked SO for our study because SO is one of the most popular online software forums for developers to 
%discuss about diverse topics related to software development~\cite{Uddin-SurveyOpinion-TSE2017,Ponzanelli-PrompterRecommender-EMSE2014}. 
%SO produces a full dump of all the posts (questions and answers) every quarter. 
We download the SO data dump~\cite{website:stackoverflow-datadump} 
of September 2019, which is the latest dump available during the time of analysis. 
%We produce our dataset for the study using the dump instead of live SO API to 
%ensure a static reference point of our study for future 
%extension (e.g., reproducibility). 
Each post contains the following meta information: \begin{inparaenum}
\item Post textual contents and code examples, 
\item Post creation and edition times,
\item Post score, favorite and view counts,
%\item If the post is an answer, 
\item The user who created the post, and
\item If it is a question, the user provided tags given to the post.
\end{inparaenum} An answer to a question is flagged as accepted, if the user 
who has asked the question marked the answer as accepted. A question can have between 1 and 5 tags.
The SO  dataset includes all posts for 11 years between 2008 
and September 2019.  In total, it has 46,767,375 questions and answers. 
Out of those around 40\% are questions and 60\% are answers. 
Out of the answers, around 34\% are accepted. 
%A total of 11,337,789 users participated in the discussions. %(i.e., asked questions/answered/commented). 

\nd\bf{\ul{Step 2. Develop IoT Tag Set.}} 
%We use the user-defined
%IoT tags given to the questions. However, not all the tags can be related to the IoT discussions. 
To determine the list of potential IoT tags in SO, we adapt the following approach based on Yang et al.~\cite{YangLo-SecurityDiscussionsSO-JCST2016}.
\begin{inparaenum}[(1)]%[label=2(\alph*),leftmargin=15pt]
  \item {Identify Initial IoT Tags.} We identify three most popular IoT related tags in SO. We denote those $\mathcal{T}_{init}$.
  \item {Determine Final IoT Tags.} We collect candidate tags related to $\mathcal{T}_{init}$ by analyzing tags that show significant relevance 
  with tags in $\mathcal{T}_{init}$. The final list $\mathcal{T}_{final}$ contains 78 candidate tags. 
  %\tbl\ref{tab:tagsUsed} lists the tags from $\mathcal{T}_{init}$ and $\mathcal{T}_{final}$. 
\end{inparaenum} We discuss each step below.

\begin{inparaenum}[(1)]
\item\ib{Identify Initial IoT Tags.} Intuitively, a significant number of IoT related posts in SO could be labeled as tags having the keyword `iot'. 
On September 2019, we thus searched for the `iot' tagged posts. The SO search engine returned posts tagged as `iot' and a list of 
top 20 tags relevant to `iot', such as `raspberry-pi', `arduino', `windows-10-iot-core', `python', etc. 
The relevant tags are most frequently co-occurred in the `iot' tagged posts. The 20 relevant tags 
can be broadly be categorized into two types: \begin{inparaenum}
\item Tags with `iot' suffix/prefix (e.g., windows-iot), 
\item Tags related to the usage of two (Arduino and raspberry) predominantly used IoT technologies and their various incarnations and usage across domains and cloud (e.g, homekit),  
%\item IoT Platform and/or SDK: raspberry-pi, azure-iot-hub, arduino, aws-iot, windows-iot-core, raspberry-pi3, 
%\item Language: C\#,  python, java, node.js, 
%\item Network/Communication: mqtt, esp8266, javascript, node-red, and
%\item Others: azure, amazon-web-services, ibm-cloud, android,  windows, uwp. 
\end{inparaenum} 
%Besides the first category (i.e., IoT Platform and/or SDK), the other tags are generic. For example, if a question is tagged as `python', it can be any discussion related to 
%Python programming language that may not necessarily related to IoT. However, if such a tag is accompanied by `iot' or any any IoT platform or SDK related tag in a post, 
%the post should contain discussion about IoT. 
We thus consider the following three 
tags as $\mathcal{T}_{init}$: \begin{inparaenum}
\item iot or any tag with `iot' keyword, e.g., `azure-iot-hub', 
\item arduino, and 
\item raspberry-pi.
\end{inparaenum} Besides the iot tags, arduino and raspberry-pi are the two most popular open source 
platforms to develop IoT based applications (with dedicated SDKs). Both platforms 
have undergone rapid evolution through multiple versions, such as raspberry-pi, raspberry-pi2, etc.        

\item\ib{Determine Final IoT Tags.} Intuitively, besides the three tags in $\mathcal{T}_{init}$, there 
can be other potential IoT-related tags in SO that developers \it{frequently} use to tag 
IoT-related questions. We identify those other potential tags as follows. 
Suppose, the entire SO data dump is denoted as $\mathcal{D}$. 
First, we start the tag set in $\mathcal{T}_{init}$ that are obvious candidates to find posts related to IoT discussions. Second, 
we extract a list of all questions $\mathcal{P}$ from our dataset that are labeled at least one of those tags in $\mathcal{T}_{init}$. 
Third, we extract the list of all tags $\mathcal{T_A}$ from $\mathcal{Q}$. Not all the tags in $\mathcal{A}$ may correspond to IoT (e.g., python). 
Therefore, following previous research~\cite{YangLo-SecurityDiscussionsSO-JCST2016,Bagherzadeh-BigdataTopic-FSE2019} 
we systematically filter out \it{irrelevant} tags and 
finalize a list of all potential IoT tags $\mathcal{T}$ 
from $\mathcal{A}$ as follows. For each tag $t$ in $\mathcal{T_A}$, we compute its significance and relevance 
with regards to $\mathcal{P}$ (i.e., questions tagged as the $\mathcal{T}_{init}$) and $\mathcal{D}$ (i.e, entire SO dataset) 
as follows.  
\begin{equation}
\textrm{Significance}~\mu(t) = \frac{\# \textrm{of Questions with tag $t$ in $\mathcal{P}$}}{\# \textrm{of Questions with tag $t$ in $\mathcal{D}$}}
\end{equation}
\begin{equation}
\textrm{Relevance}~\nu(t) = \frac{\# \textrm{of Questions with tag $t$ in $\mathcal{P}$}}{\# \textrm{of Questions in $\mathcal{P}$}}
\end{equation}
A tag $t$ is significantly relevant to IoT discussions if $\mu(t)$ and $\nu(t)$ are higher than a specific threshold. 
Our 49 experiments with a 
broad range of threshold values of $\mu$  and $\nu$ %$\mu = \{0.05, 0.1, 0.15, 0.2, 0.25, 0.3, 0.35\}$ and $\nu = \{0.001, 0.005,
%0.01, 0.015, 0.02, 0.025, 0.03\}$ 
show that $\mu = 0.3$ and $\nu = 0.001$ allow for more 
relevant set of IoT tags. The threshold values  are consistent with 
previous work~\cite{YangLo-SecurityDiscussionsSO-JCST2016,Ahmed-ConcurrencyTopic-ESEM2018,Bagherzadeh-BigdataTopic-FSE2019}. 
\end{inparaenum} The final list of IoT-related tags is as follows.
% \begin{description}
% \item [$\mathcal{T_{\text{arduino}}}$ = ] \{
% arduino,
%   arduino-c++,
%   arduino-due,
%   arduino-esp8266,
%   arduino-every,
%   arduino-ide,
%   arduino-mkr1000,
%   arduino-ultra-sonic,
%   arduino-uno,
%   arduino-uno-wifi,
%   arduino-yun,
%   platformio\}
% \item [$\mathcal{T_{\text{iot}}}$ = ] \{audiotoolbox',
%   audiotrack,
%   aws-iot,
%   aws-iot-analytics,
%   azure-iot-central,
%   azure-iot-edge,
%   azure-iot-hub,
%   azure-iot-hub-device-management,
%   azure-iot-sdk,
%   azure-iot-suite,
%   bosch-iot-suite,
%   eclipse-iot,
%   google-cloud-iot,
%   hypriot,
%   iot-context-mapping,
%   iot-devkit,
%   iot-driver-behavior,
%   iot-for-automotive,
%   iot-workbench,
%   iotivity,
%   microsoft-iot-central,
%   nb-iot,
%   rhiot,
%   riot,
%   riot-games-api,
%   riot.js,
%   riotjs,
%   watson-iot,
%   windows-10-iot-core,
%   windows-10-iot-enterprise,
%   windows-iot-core-10,
%   windowsiot,
%   wso2iot,
%   xamarin.iot\}
% \item [$\mathcal{T_{\text{raspberry-pi}}}$ = ] \{adafruit,
%   android-things,
%   attiny,
%   avrdude,
%   esp32,
%   esp8266,
%   firmata,
%   gpio,
%   hm-10,
%   home-automation,
%   intel-galileo,
%   johnny-five,
%   lora,
%   motordriver,
%   mpu6050,
%   nodemc,
%   omxplayer,
%   raspberry-pi,
%   raspberry-pi-zero,
%   raspberry-pi2,
%   raspberry-pi3,
%   raspberry-pi4,
%   raspbian,
%   serial-communication,
%   servo,
%   sim900,
%   teensy,
%   wiringpi,
%   xbee\}
% \end{description}
% The final list of tags is a union of all candidates tags:
% \begin{equation*}
% \text{Final tags, }\mathcal{T} = \mathcal{T_{\text{arduino}}}\bigcup \mathcal{T_{\text{iot}}}\bigcup \mathcal{T_{\text{raspberry-pi}}}
% \end{equation*}
The final list of tags is a union of all 78 candidates tags that also includes the three tags in $\mathcal{T}_{init}$ (i.e., iot, arduino, raspberry-pi). 
The 78 tags 
cover a wide range technologies and services supporting the emerging IoT ecosystems in software development. 
%The services from major software vendors are offered by their IoT-platforms, 
%e.g., windowsiot and azure-iot from Microsoft, watson-iot from IBM, google-cloud-iot from Google, aws-iot from Amazon, and so on. 
%A variety of IoT-based network technologies can be seen in the tags, such as lora, xbee. The IoT ecosystem is 
%supported by serveral notable platforms and SDKs, as evidenced by the tags (johny-five, raspian, attiny, etc.).
%Our replication package lists all 78 IoT tags.
 
%\gias{provide justification that the 78 tags contain IoT discussions}

\nd\bf{\ul{Step 3. Download IoT Posts.}} Our final dataset consists of all posts tagged as at least one 
of the candidate 78 tags. A SO question is an IoT question if it is tagged one or more of the 
tags from $\mathcal{T}$. Based on the 78 tags, we found a total of 81,651 posts (questions and answers) in our SO dump, 
out of which around 48\% are questions (i.e., 39,305) and 52\% (42,346) are answers. Out of the answers, around 
33\% (13,868) are accepted. Following previous
research~\cite{Bagherzadeh-BigdataTopic-FSE2019,Barua-StackoverflowTopics-ESE2012,Rosen-MobileDiscussionSO-EMSE2016},
we only consider the questions and accepted answers to the questions.
%Unaccepted answers to each question are not considered to avoid noise.
Our final dataset $\mathcal{B}$ consists of a total of 53,173 posts (39,305 questions, 13,868 accepted answers).

\subsection{Creation of IoT Security Aspect Benchmark}
We sampled 1984 sentences from 53K posts. We labeled them. Discuss the cohen kappa agreement.


==> detectIoTSecurity.tex <==
\section{Automatic Detection of IoT Security Aspect}\label{sec:results-aspect-detection}
We answer four research questions during our investigation on the effectiveness of deep learning models to detect security aspects in developer discussions:
\begin{enumerate}[leftmargin=30pt, label=\bf{RQ\arabic{*}.}]
%  \item How do the deep learning models perform to detect security aspects in Opiner API review dataset? (\sec\ref{sec:performance-api-review-dataset})
  %\item Can the advanced transfoer models offer improved performance to detect security aspects in Opiner benchmark? (\sec\ref{sec:rq-bert-opiner-data})
%  \item Can the models trained on API review dataset show similar performance in IoT discussions?  (\sec\ref{sec:rq-secbot-assess-iot})
  %\item Can the models be further improved by re-training on labeled data from IoT security discussions? (\sec\ref{sec:rq-secbotplus-dev})
  \item How do the deep learning models perform to detect IoT security aspects in the benchmark?
  \item What are the error categories in the misclassified cases of the best performing model? (\sec\ref{sec:misclassification-analysis-secbot+})
  %\item Can the Performance of the BERT-Models Be Further Improved Using SE-Specific Embedding? 
\end{enumerate}
The answer to first research question (RQ1) helps us to determine whether deep learning models can outperform the shallow learning models in Opiner for an already available 
benchmark dataset of API review aspects. The API review dataset in Opiner does not have any sentences/posts picked from our 53K IoT posts. 
While security discussions are prevalent across diverse computing paradigms, the nature of their discussions (e.g., the vocabularies, contexts) could 
differ between and among the domains. The second research question (RQ2) then attempts to find out whether security aspect classification model trained on API review 
dataset can perform well to detect security discussions in our IoT dataset. Intuitively, a good performance in such cross-data setting denote that security discussions 
follow similar patterns between the two IoT and non-IoT (e.g., API review dataset) datasets in our study. The third research question (RQ3) aims to answer 
whether and how by adding IoT-specific security discussions into the API review dataset would offer improved performance for the security aspect detection models. 
The last research question (RQ4) offers a qualitative perspective on the misclassifications of the best performing classification model by analyzing the error categories. 
Such analysis can help determine the causes of misclassifications and possible venues of further improvement in the security aspect detection in IoT developer discussions.    
\subsection{Performance Metrics} \label{sec:performance-metrics}
We analyze the performance of the classification models for security aspect detection using five standard metrics in 
information retrieval~\cite{Manning-IRIntroBook-Cambridge2009}: Precision (P), Recall (R), F1-score (F1), Accuracy (Acc) and Area Under the Curve (AUC).
\begin{itemize}[leftmargin=20pt]
  \item Precision (P) is the fraction of sentences labeled `HasSecurity' (i.e., the sentence contains security discussions) out of all the sentences labeled as `HasSecurity'. 
  \begin{equation}
  P  = \frac{TP}{TP+FP}
  \end{equation}
Here TP = Correctly classified a sentence as containing discussion about security, FP = Incorrectly classified as containing discussion about security,   
  \item Recall (R) is the fraction of all `HasSecurity' sentences that are successfully identified out of all sentences that contain security discussions.
  \begin{equation}
	R = \frac{TP}{TP+FN}
  \end{equation}
  Here FN = Incorrectly classified as not containing discussion about security.
  \item F1-score is the harmonic mean of precision (P) and Recall (R). 
  \begin{equation}
	F1 = 2*\frac{P*R}{P+R}
  \end{equation}
  \item Accuracy (A) is the fraction of all correctly classified out of all records.
  \begin{equation}
	Acc = \frac{TP + TN}{TP + TN + FP + FN}
  \end{equation}
  Here TN = Correctly classified as not containing discussion about security.
  \item AUC (Area Under the Curve) is the area under the Receiver Operating Characteristics (ROC) curve. An ROC curve is a graphical plot to illustrate the ability of a binary classifier (such as ours) 
  The ROC curve is plotted by taking ratio of TPR (True Positive Rate) against FPR (False Positive Rate) at various classification probability threshold (e.g., a probability of 1.0 will most likely denote a 
  100\% TPR and 0\% FPR, while a probability of 0.0 will most likely result the opposite). We calculate TPR and FPR and use those to calculate AUC as follows . 
  \begin{eqnarray}
  TPR = \frac{TP}{TP + FN}, ~
  FPR = \frac{FP}{FN + TP}, ~
  AUC = \int_{x = 0}^{1} {TPR}({FPR}^{-1}(x))dx
  \end{eqnarray}
  %\item MCC  
\end{itemize}
F1-score and AUC are preferred over metrics like accuracy (A) when evaluation dataset is imbalanced. For example, 
our API review dataset is imbalanced with lower number of sentences labeled as 1 (i.e., `HasSecurity' = 1) than sentences labeled as 0.  
Following standard practices in Literature~\cite{Zhang-SentimentDetectionSEBERT-ICSME2020,Uddin-OpinionValue-TSE2019}, 
we use F1-score to determine and report the best model. 



% 
% \begin{table}[t]
%   \centering
%   \caption{Summary stats for Opiner Dataset}
%     \begin{tabular}{rrrr}\toprule
%     \midrule
%     {\textbf{Total T}} & {\textbf{\#Security S}} & {\textbf{\%S/T}} & {\textbf{Non-Security}} \\
%     \midrule
%     4297  & 163   & 3.8\% & 4134 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:opiner-details}%
% \end{table}%


% 
% 
% In Machine Learning, dataset is divided into two or three subsets, training,
% validation, and testing. Model is trained on training dataset, tuned on
% validation dataset, and tested on testing dataset. Mainly, testing and
% validation dataset are used to limit model from getting overfitted and tuning
% the hyperparameters respectively. This strategy works fine when dataset is large
% but often struggles when dataset is small as training instances are deficient
% compared to model's parameters and thus, model underfits. Model needs
% substantial training data to overcome underfitting and at the same time,
% validation data to find the best parameter as well as best model, and also
% testing dataset to eschew underfitting. We need a middle ground, which seems a
% bit contradictory as well, where all requirements are met without compromising.
% Here comes $k-fold~cross~validation$\cite{inproceedings} to rescue. The idea is
% to divide the dataset, $D$, into $k$ disjoint folds, $D_i,~i=1...k$, of
% approximately equal size.
% $$D_i\cap D_j=\phi~~~\forall~i,j\in k~and ~i\ne j $$
% $$D_1\cup D_2\cup...\cup D_k = D$$
% To avoid overfitting, model is trained $k$ times, each time one of the $k$ folds are held out as validation set and rest of the $k$ folds are used as training set. The value of $k$ is a hyperparameter. This technique is quite effective in learning with small balanced dataset but could suffer from undersampling if dataset is imbalanced, like ours. Stratified random sampling, equally divides dataset into homogeneous subsets before sampling, can overcome the undersampling problem. Thus, we used \textbf{stratified} $k-fold~cross~validation$. We set \textbf{k as 10}, a value that has been found through experiment.\\
% 


\subsection{Performance of Deep Learning Models on API Review Dataset (RQ1)}\label{sec:performance-api-review-dataset}
We investigate whether deep learning models like seq2seq and transformer models from \sec\ref{sec:studied-models} 
can outperform the two shallow learning models for security aspect detection in Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019}. 
\subsubsection{Approach}\label{sec:opiner-dataset-performance-approach} We use the API review dataset 
from \sec\ref{sec:studied-datasets} for the investigation. 
For experimentation, similar to Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019}, we use a k-fold cross-validation ( k = 10). 
Thus, we used stratified k-fold cross validation., each fold divides dataset $D$ into $k$ disjoint folds, each of
approximately equal size.
$D_i\cap D_j=\phi~~~\forall~i,j\in k~and ~i\ne j $ and 
$D_1\cup D_2\cup...\cup D_k = D$. To avoid overfitting, model is trained $k$ times, each time one of the $k$ folds
are held out as validation set and rest of the $k$ folds are used as training
set. The value of $k$ is a hyperparameter. This technique is quite effective in
learning with small balanced dataset but could suffer from under sampling if
dataset is imbalanced, like ours. Stratified random sampling, equally divides
dataset into homogeneous subsets before sampling, can overcome the under sampling
problem. For the two baselines (Logit and SVM), we hyper tuned all the parameters used by Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017}. 
In addition to Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017}, we also set the random\_state value as 42 to 
ensure determinism of the results among multiple runs. 
 

\begin{table}[t]
\centering
\caption{Hyperparameters of the deep learning models on the API review dataset}
\begin{tabular}{p{2cm}l|rrrrr}
\toprule
\bf{Type} & \textbf{Model}& \bf{Batch Size} & \bf{Epochs}  & \bf{Optimizer} & \bf{Loss Functions} & \bf{Learning Rate}\\ 
\midrule
\multirow{2}[0]{*}{seq2seq} &  LSTM & 64 & 50 & Adam & binary-crossentropy & 2e-3\\ 
& Bi-LSTM & 64 & 20 & Adam & binary-crossentropy & 2e-3\\
 \midrule
\multirow{5}[0]{*}{Transformer} & BERT & 32 & 3 & Adam & binary-crossentropy & 3e-5 \\
& RoBERTa & 32 & 3 & Adam & binary-crossentropy & 1e-5 \\
& XLNet & 32 & 3 & Adam & binary-crossentropy & 3e-5 \\
& ALBERT & 32 & 3 & Adam & binary-crossentropy & 1e-5 \\
& DistilBERT & 16 & 3 & Adam & binary-crossentropy & 3e-5\\
 %FunnelBERT & funnel-transformer/small-base &12& 768 & 12 & 115M \\
 %ELECTRA& google/electra-small-discriminator&  12&	256&12 &	14M\\
\bottomrule
\end{tabular}
%}
\label{dllParamAPIReview} 
%\end{center}
\end{table}
% \begin{table}[t]
% \centering
% \caption{Hyperparameters of BERT variants}
% \begin{tabular}{l|c|c|rrr}
% \toprule
% \textbf{Model}& \bf{Optimizer} & \bf{Loss Functions} & \bf{Batch Size} & \bf{Epochs}   & \bf{Learning Rate}\\ 
% \midrule
%  BERT & \multirow{5}[0]{*}{Adam} & \multirow{5}[0]{*}{binary-crossentropy} & 32 & 3 & 3e-5\\ 
%  RoBERTa &   &&32 & 3 & 1e-5\\
%  XLNet &  &&32 & 3  & 3e-5\\
%  ALBERT &  &&32 & 3  & 1e-5\\
%  DistilBERT &&&  16 & 3 & 3e-5\\
%  %FunnelBERT & funnel-transformer/small-base &12& 768 & 12 & 115M \\
%  %ELECTRA& google/electra-small-discriminator&  12&	256&12 &	14M\\
% \bottomrule
% \end{tabular}
% %}
% \label{BERT Hyperparameters} 
% %\end{center}
% \end{table}

For each deep learning model, following literature in text classifications~\cite{Alharbi-LSTM-CognitiveJournal2019,Hameed-BiLSTM-IEEEAccess2020,Delvin-BERTArch-Arxiv2018}, 
we tuned the following hyperparameters for optimal 
performance: \begin{inparaenum}[(1)]
\item Batch size, 
\item Number of hidden layers, neurons, units, filters, epochs 
\item Optimizer, Activation, and loss functions, and
\item Learning rate.
\end{inparaenum} We tune these hyparparameters using standard Grid search technique~\cite{random-search}. 
In \tbl\ref{dllParamAPIReview}, we show the values of selected hyperparameters in our deep learning model after tuning.  
Our replication package details the hyperparameter values with source code. %that used the hyperparameter for the experimentation.
% Based on hyperparameter tuning, we find the following configurations worked 
% best for the models in the benchmark: \begin{inparaenum}[(1)]
% \item DNN: batch size = 128, \#hidden layers = 1, \#neurons = 64, 
% optimizer= Adam, activation function=ReLU, epochs=20, prediction function=sigmoid, loss=binary cross-entropy, 
% \item CNN: batch size = 128, \#filters = 256, kernel size=3, pool size=3, optimizer=Adam, activation function=ReLU, learning rate = 2e-3, prediction function=sigmoid, epochs=20, loss=binary cross-entropy, 
% \item LSTM: batch size = 128, units size=64,optimizer=Adam, activation function=ReLU,learning rate = 2e-3,epochs=20, prediction function=sigmoid, loss=binary cross-entropy,
% \item Bi-LSTM: batch size = 16, optimizer=Adam, learning rate = 3e-5, epochs=3, loss=spare categorical cross-entropy.   
% \end{inparaenum}
% 
% 
% {Hyperparameters for SGDClassifier: alpha=.0001, max\_iter=2000,epsilon=0.5, loss='log',penalty="l2",power\_t=0.5, warm\_start=False, shuffle=True, class\_weight='balanced'\\
% Hyperparameters for Logistic Regression: max\_iter=2000,penalty='l2',warm_start=False,class\_weight='balanced'\\
% I used random\_state=42 for Stratified K Fold validation\\
% for feature vector: sublinear\_tf=True, max\_df=.5, stop\_words='english'\\
% }

% \begin{table}
% \caption{Performance of traditional DL models on benchmark~\cite{Uddin-OpinionValue-TSE2019}}
%  \begin{tabular}{l|lrrrrr}\toprule 
% 
%  \bf{Model} & \bf{P} & \bf{R} & \bf{F1} & \bf{AUC} & \bf{MCC} \\ \midrule
%  LSTM & \\
%  Bi-LSTM & \\
% %  Bags of words & Baseline - Logit &0.67 & 0.77 & 0.72\\
% %  Bag of words & Baseline - SVM &0.69 & 0.77 & 0.73 \\
%   \midrule
%  \multicolumn{7}{c}{Performance Change in \% of Bi-LSTM over Baseline Opiner~\cite{Uddin-OpinionValue-TSE2019}}\\
%  \midrule
% %   Bag of words & Baseline - Logit & 6.9\%$\uparrow$ & -20.3\% $\downarrow$ & -5.9\%$\downarrow$ \\
% %  Bag of words & Baseline - SVM & 4.2\%$\uparrow$ & -20.3\% $\downarrow$ & -7.4\%$\downarrow$ \\
%  
%  \bottomrule
% \end{tabular}
%     
%     \label{tab:dnn_performance}
% \end{table}


% \begin{table}
% \caption{Combined}
%  \begin{tabular}{l|lrrrrr}\toprule 

%  \bf{Feature} & \bf{Model} & \bf{P} & \bf{R} & \bf{F1} & \bf{AUC} & \bf{MCC} \\ \midrule
%  Bag of words &DNN & 0.87 & 0.691 & 0.77 & 0.839 & 0.749\\
 
%  GloVe (200D) & CNN & 0.882 & 0.775 & 0.821 & 0.879 & 0.802\\
%  GloVe (200D) &LSTM & 0.866 & 0.861 & 0.861 & 0.92 & 0.842 \\
%  GloVe (200D)  & Bi-LSTM & 0.861 & 0.849 & 0.854 & 0.914 & 0.833\\
% %  Bags of words & Baseline - Logit &0.67 & 0.77 & 0.72\\
% %  Bag of words & Baseline - SVM &0.69 & 0.77 & 0.73 \\
%   \midrule
%  \multicolumn{7}{c}{Performance Change in \% of Bi-LSTM over Baseline Opiner~\cite{Uddin-OpinionValue-TSE2019}}\\
%  \midrule
%   Bag of words & Baseline - Logit & 6.9\%$\uparrow$ & -20.3\% $\downarrow$ & -5.9\%$\downarrow$ \\
%  Bag of words & Baseline - SVM & 4.2\%$\uparrow$ & -20.3\% $\downarrow$ & -7.4\%$\downarrow$ \\
 
%  \bottomrule
% \end{tabular}
    
%     \label{tab:dnn_performance}
% \end{table}

% Table generated by Excel2LaTeX from sheet 'RQ1'
% Table generated by Excel2LaTeX from sheet 'RQ1'
\begin{table}[t]
  \centering
  \caption{Performance of security aspect detection of deep seq2seq and shallow learning models in the API review dataset~\cite{Uddin-OpinionValue-TSE2019}}
    \begin{tabular}{llrrrrr}\toprule
    \textbf{Model Type} & \textbf{Model Name} & {\textbf{P}} & {\textbf{R}} & {\textbf{F1}} & {\textbf{Acc}} & {\textbf{AUC}} \\
    \midrule
    Baseline Shallow & SVM   & 0.684 & 0.76  & 0.713 & 0.978 & 0.873 \\
          & Logit & 0.682 & 0.796 & \textbf{0.728} & 0.978 & 0.891 \\
          \midrule
    seq2seq & LSTM (100D)  & 0.703 & 0.7   & \textbf{0.698} & 0.977 & 0.844 \\
          & Bi-LSTM (200D) & 0.722 & 0.582 & 0.63  & 0.976 & 0.786 \\
          \midrule
    \multicolumn{7}{c}{\bf{Performance Change in LSTM Over Baselines}} \\
    \midrule
    \multicolumn{2}{c}{Over SVM} & 2.8\% & -7.9\% & -2.1\% & -0.1\% & -3.3\% \\
    \multicolumn{2}{c}{Over Logit} & 3.1\% & -12.1\% & -4.1\% & -0.1\% & -5.3\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:modelPerformanceSeq2SeqAPIReviewDataset}
\end{table}%
\begin{table}[t]
  \centering
  \caption{Performance of security aspect detection of deep transformer models in the API review dataset~\cite{Uddin-OpinionValue-TSE2019}}
    \begin{tabular}{llrrrrr}\toprule
    \textbf{Model Type} & \textbf{Model Name} & {\textbf{P}} & {\textbf{R}} & {\textbf{F1}} & {\textbf{Acc}} & {\textbf{AUC}} \\
    \midrule
    Transformer & BERT  & 0.722 & 0.808 & 0.733 & 0.981 & 0.896 \\
          & RoBERTa & 0.742 & 0.871 & \textbf{0.794} & 0.984 & 0.929 \\
          & XLNet & 0.686 & 0.809 & 0.728 & 0.979 & 0.896 \\
          & ALBERT & 0.775 & 0.724 & 0.737 & 0.982 & 0.857 \\
          & DistilBERT & 0.764 & 0.76  & 0.727 & 0.982 & 0.874 \\
    \midrule
    \multicolumn{7}{c}{\bf{Performance Change in RoBERTa Over Baselines \& LSTM}} \\
    \midrule
    \multicolumn{2}{c}{Over SVM} & 8.5\% & 14.6\% & 11.4\% & 0.6\% & 6.4\% \\
    \multicolumn{2}{c}{Over Logit} & 8.8\% & 9.4\% & 9.1\% & 0.6\% & 4.3\% \\
    \multicolumn{2}{c}{Over LSTM (100D)} & 5.5\% & 24.4\% & 13.8\% & 0.7\% & 10.1\% \\

    \bottomrule
    \end{tabular}%
  \label{tab:modelPerformanceBERTAPIReviewDataset}
\end{table}%


\subsubsection{Results} In \tbl\ref{tab:modelPerformanceSeq2SeqAPIReviewDataset}, we report the performance of the two baselines (SVM and Logit) and the two Seq2Seq deep learning 
models (LSTM and Bi-LSTM) to detect security aspect on the Opiner API review dataset~\cite{Uddin-OpinionValue-TSE2019}. For each 
model, we report five performance metrics from \sec\ref{sec:performance-metrics}. The last two rows in \tbl\ref{tab:modelPerformanceSeq2SeqAPIReviewDataset} shows 
the performance change (in percentages) we observed in the best performing seq2seq model (LSTM) compared to the two baselines. 

Among the two 
shallow learning baselines, Logit shows the best F1-score of 0.728, while SVM shows and F1-score of 0.713. We note that both of these F1-scores are higher than the F1-scores of the two models reported by Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017}. 
For example, Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017} reported an F1-score of 0.60 for both SVM and Logit. The higher 
performance in our experiment for both models is due to the following reasons: \begin{inparaenum}[(1)]
\item The removal of 225 duplicate sentences has reduced skewness of the benchmark dataset and made it more balanced, and
\item Given Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017} used 10-fold cross-validation, the duplicates 
have unexpectedly changed the weights of the model parameters, introducing underfitting or overfitting in the resulting model while training.  
\end{inparaenum}   

\begin{figure}
\hspace*{-8cm}
\begin{tikzpicture}
\begin{axis}[
    title = {LSTM},
    xlabel={Glove Dimensions},
    xmin=50, xmax=200,
    ymin=0, ymax=1,
    xtick={50,100,150,200},
    ytick={.25,.5,.75,1},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (50,0.771)(100,0.844)(200,0.818)
    };
    \addlegendentry{AUC}
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (50,0.601)(100,0.698)(200,0.676)
    };
    \addlegendentry{F1-Score}
\end{axis}
\hspace{8cm}
\begin{axis}[
    title = {Bi-LSTM},
    xlabel={Glove Dimensions},
    xmin=50, xmax=200,
    ymin=0, ymax=1,
    xtick={50,100,150,200},
    ytick={.25,.5,.75,1},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
]
\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (50,0.768)(100,0.775)(200,0.786)
    };
    \addlegendentry{AUC}
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (50,0.608)(100,0.622)(200,0.630)
    };
    \addlegendentry{F1-Score}
    
\end{axis}

\end{tikzpicture}
\caption{Change in F1 and AUC scores in LSTM and Bi-LSTM based on Glove word embedding dimensions}
\label{fig:changeInScoreByWordDimensionLSTMBiLSTM}
\vspace{-3mm}
\end{figure}



% \pgfplotsset{width=10cm}
% \begin{figure}
% \hspace*{-5cm}
% \begin{tikzpicture}
% \begin{axis}[
%     title = {RoBERTa},
%     xlabel={FPR},
%     ylabel = {TPR},
%     xmin=0, xmax=1,
%     ymin=0, ymax=1,
%     xtick={0,0.05,0.1,.2,0.3,.4,0.5,.6,.7,.8,.9,1},
%     ytick={0,0.05,0.1,.2,0.3,.4,0.5,.6,.7,.8,.9,1},
%     legend pos=south east,
%     ymajorgrids=true,
%     grid style=dashed,
% ]
% 
% \addplot[
%     color=green,
%     ]
%     coordinates {
%     (0.0, 0.0)
% (0.0, 0.0981012658227848)
% (0.0, 0.4208860759493671)
% (0.0014970059880239522, 0.5031645569620253)
% (0.005988023952095809, 0.7215189873417721)
% (0.01347305389221557, 0.8164556962025317)
% (0.025449101796407185, 0.8386075949367089)
% (0.03293413173652695, 0.8544303797468354)
% (0.07634730538922156, 0.8670886075949367)
% (0.10029940119760479, 0.8829113924050633)
% (0.1092814371257485, 0.8860759493670886)
% (0.12874251497005987, 0.9050632911392406)
% (0.1661676646706587, 0.9208860759493671)
% (0.16766467065868262, 0.930379746835443)
% (0.19610778443113772, 0.9367088607594937)
% (0.19910179640718562, 0.9430379746835443)
% (0.22005988023952097, 0.9462025316455697)
% (0.25898203592814373, 0.9525316455696202)
% (0.27395209580838326, 0.9588607594936709)
% (0.2754491017964072, 0.9683544303797469)
% (0.2844311377245509, 0.9715189873417721)
% (0.3083832335329341, 0.9810126582278481)
% (0.3203592814371258, 0.9873417721518988)
% (0.3532934131736527, 0.990506329113924)
% (0.3712574850299401, 0.9968354430379747)
% (0.9356287425149701, 1.0)
%     };
%     \addlegendentry{ROC}
% \addplot[
%     color=red,
%     % mark=square,
%     ]
%     coordinates {
%     (0,0)(1,1)
%     };
%     \addlegendentry{Random guess}
% \end{axis}
% \end{tikzpicture}
% \caption{Change in F1 and AUC scores in LSTM and Bi-LSTM based on Glove word embedding dimensions}
% \label{fig:changeInScoreByWordDimensionLSTMBiLSTM}
% \vspace{-3mm}
% \end{figure}
% 


In terms of F1-score, none of the seq2seq DL models manage to outperform the 
the two shallow learning baselines in \tbl\ref{tab:modelPerformanceSeq2SeqAPIReviewDataset}. The best learning seq2seq model was LSTM with an F1-score of 0.676, followed by 
bi-LSTM with an F1-score of 0.630. We report the performance of LSTM for 100 Glove dimension and of Bi-LSTM for 200 Glove dimension. The two models 
showed the best F1-score for the two dimensions. In \fig\ref{fig:changeInScoreByWordDimensionLSTMBiLSTM}, we show the change in F1 and AUC scores of the 
LSTM and Bi-LSTM as we change the Glove word dimension. We checked for all available Glove word dimensions (starting from 50) available in the 
huggingface package. While for Bi-LSTM the maximum F1 and AUC score reached at 200 dimension, the scores are still substantially lower than those of 
LSTM. We, therefore, considered that Bi-LSTM cannot outperform LSTM even with  higher dimension. Indeed, at 300 word dimension, which is the maximum availble 
dimension in Glove, Bi-LSTM showed an F1-score 0.660 compared to the best F1-score of 0.698 at 100 dimension.    


In \tbl\ref{tab:modelPerformanceBERTAPIReviewDataset}, we report the performance of the five advanced lagnuage-based pre-trained transformer 
models  on the API review datasets: BERT, RoBERTa, XLNet, ALBERT, and DistilBERT. The last three rows in \tbl\ref{tab:modelPerformanceSeq2SeqAPIReviewDataset} shows 
the performance change (in percentages) we observed in the best performing transformer model (RoBERTa) compared to the two baselines from Opiner (SVM and Logit) and the 
best performing seq2seq model from \tbl\ref{tab:modelPerformanceSeq2SeqAPIReviewDataset} (i.e., LSTM). The low performnace of  
Bi-LSTM compared to LSTM could be attributed to the fact that Bi-LSTM takes both words and their bidirectional sequence into consideration 
to learn about structure. For security aspects, classifications can be often more straightforward, i.e., a parsing of past to future could 
suffice (e.g., secure and stable connection), while a future to past parsing may not offer much benefit but may instead confuse the classifier with redundant contexts. 


Three of the five transformer models (BERT, RoBERTa, and Albert) outperform all the baselines and seq2seq models in terms of F1-scores. The best 
performing transformer model is RoBERTa with an F1-score of 0.794, which outperfoms the baselines SVM by 11.4\%, Logit by 9.1\% and the LSTM (100D) by 13.8\%. 
The superiority of the three models (BERT, RoBERTa, and Albert) over the seq2seq models and baselines is not surprising given that 
the three transformer models are generally found to have offered better performance than state-of-the-art classifiers for multiple other 
text classification tasks in software engineering (e.g., sentiment detection~\cite{Zhang-SentimentDetectionSEBERT-ICSME2020}). We refer to the 
best performing transformer model, RoBERTa, as \bf{\ul{SecBot}} in the remainder of the paper. 

% In \tbl\ref{tab:dnn_performance}, we report the performance of the four DL models and the two shallow learning baselines (SVM and Logit) on 
% Opiner benchmark~\cite{Uddin-OpinionValue-TSE2019}. In terms of F1-score, none of the four traditional DL models manage to outperform the 
% the two shallow learning baselines. SVM shows the best performance with an F1-score of 0.73, while Logit shows the second best performance with an F1-score of 0.72. 
% We note that both of these F1-scores are higher than the F1-scores of the two models reported by Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017}. 
% For example, Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017} reported an F1-score of 0.60 for both SVM and Logit. The higher 
% performance in our experiment for both models is due to the following reasons: \begin{inparaenum}[(1)]
% \item The removal of 225 duplicate sentences has reduced skewness of the benchmark dataset and made it more balanced, and
% \item Given Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017} used 10-fold cross-validation, the duplicates 
% have unexpectedly changed the weights of the model parameters, introducing underfitting or overfitting in the resulting model while training.  
% \end{inparaenum} 

% Among the DL models, the best performing models are Bi-LSTM and LSTM. Both show an F1-score of 0.68. Thus, the two baselines Logit and SVM 
% outperform the two DL models by 5.9\% and 7.4\%, respectively. In terms of precision, DNN shows the best precision (0.81) out of all the models including the 
% DL and baselines. However, DNN suffers from low recall (0.35 compared to max 0.77 by both the baselines).  
% 
% We find that 
% Glove 200D embedding as features offered the best performance for the three models: CNN, LSTM, Bi-LSTM. \gias{do we have data for the performance of the three models using the other dimensions, e.g., 50D, 100D, 150D, 250D?} For DNN, bag 
% of words as features offered the best performance. DNN predicts positive instances precisely
% but failed to detect many positives. CNN has  higher
% precision but low reall. The use of GloVe embedding 
% offered better F1-score in LSTM and Bi-LSTM than the other two DL models (0.68 vs 0.25 in CNN and 0.49 in DNN).
% CNN also used GloVe embedding, but unlike LSTM and Bi-LSTM, CNN did not take into account information about word sequences. This means that 
% contextual information based on the relationship/dependency among words is important to detect security.
% %Both LSTM and Bi-LSTM have almost similar performance. For Bi-LSTM, we used two LSTM each having unit size of 64
% %and concatenated the outputs. Then, we fed the output to a fully connected layer
% %of 64 neurons, flattened the outputs and fed it into another fully connected
% %layer of 32 neurons before the final output layer. The use of two LSTMs offered the model to preserve contextual information better than 
% %a single LSTM model. As such, Bi-LSTM model predicted
% %more precisely than LSTM model where LSTM model explored more positive instances
% %than Bi-LSTM.   
% Overall, Bi-LSTM takes both words and their sequence into consideration 
% to learn about structure, meaning and context of the sentence. However, due to
% the low frequency of positive instances, the DL models
% failed to generalize the data properties. 
%of different classes of instances which
%resulted in misclassifications. %of many instances. 

% 
% {So, we chose our best performing model based on F1-Score
% where Bi-LSTM showed 3.86\% improvement over LSTM.} Then we comapred our best
% performing Deep Learning Model with baseline-Logit. We showed our result in
% {Table\ref{tab:dnn_performance}. Bi-LSTM led 11.42\% in Recall, 16.11\%
% in F1-Score but lagged 6.84\% in Precision. This shows Bi-LSTM exploiting more
% positive instances than Logits but surly Bi-LSTM does not predict precisely.}
% This happens because Logits model makes prediction based on words present in a
% sentence. Unseen words during validation and testing, implicit meaning of the
% sentences can hardy be understood in Logits model. On contrary, Word embedding,
% GloVe Embedding\cite{pennington-etal-2014-glove} reduces the possibilities of
% unseen data and also gives insights about context and word meaning. 
% 
% 
% 
% Overall, the lower performance of the DL models compared to the baselines is attributed to the low number of 
% positive instances (i.e., sentences labeled as security) in the benchmark. The DL models need more data to learn about the 
% word representations and to address underlying sparcity in the data. 
% One way to address the low performance issues in DL models is to increase the number of positive instances in the 
% data. Another way is to leverage the pre-trained weights of the underlying features (e.g., words/sequences) available in the recently developed 
% advanced pretrained BERT-based models. We investigate BERT~\cite{Delvin-BERTArch-Arxiv2018} based DL models in RQ2. 
%Based on this result, 
%
%we can say Deep Learning model performs better than
%shallow learning model.

% \begin{table}[t]
%   \centering
%   \caption{Summary stats and agreements for the IoT Discussion sample}
%    %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lrrr|rr}\toprule
%     \multirow{2}[0]{*}{\textbf{Sample}} & \multicolumn{3}{c}{\textbf{Summary}} & \multicolumn{2}{c}{\textbf{Agreement}} \\
%     \cmidrule{2-6}
%           & \textbf{Total T} & \textbf{\#Security S} & \textbf{\%S/T} & \textbf{Kappa} & \textbf{Percent} \\
%           \midrule
%         %IoT Training  & 1000  & 508 &  50.8\%     &   0.97     & 98.5\% \\
%         %97.7%	0.744	0.745	0.745
%     IoT Validation  & 984   &   316    & 33.1\% & 0.92     &  96.7\%  \\
%     
%     %95.8%	0.915	0.915	0.915
%     
%     % \midrule
%     % Overall $S$ & 984   &   316    &    33.1\%   & 0.92        & 96.7\% \\
%     
%     %96.7%	0.917	0.917	0.917
%     
%     
%     \bottomrule
%     \end{tabular}%
%   %}
%   \label{tab:validation-sample-stat}%
% \end{table}% 





\subsection{Performance of Models Trained using API Review Dataset on IoT Discussions (RQ2)}\label{sec:rq-secbot-assess-iot}
We assess the performance of deep learning models and baselines 
trained using API review dataset on on a validation sample of IoT developer discussions. The purpose is to determine whether 
we observe performance of the models similar to what we have observed in API review datasets. If we see differences like 
reduction in performance, we would need to re-train the models using IoT-specific developer discussions. 
% (\tbl\ref{tab:validation-sample-stat}) from the 53K IoT posts collected in \sec\ref{sec:iot-data-collection}.
 




%\subsubsection{IoT Security Benchmark} \gias{Here we report the performance of SecBot on the entire IoT security benchmark of 3000 sentences} 
\subsubsection{Approach}\sec\ref{sec:rq-secbot-assess-iot} We create a validatation dataset of 984 sentences from our IoT dataset of 53K posts. 
First, we use nltk~\cite{website:nltk} to segregate sentences from the 53K IoT posts, which 
resulted in 672,678 sentences (i.e., average 13 sentences per post). We then create our validation sample of 984 
sentences from the 672,678 sentences as follows. \begin{inparaenum}[(1)]
\item{Random Sample ($R$).} We randomly sample 384 sentences from the 672,678 sentences. This sample size is statistically significant with a 95\% confidence level and 
5 confidence interval. The first two authors then manually label each sentence as 1 (i.e., contains security discussion) 
or 0 (otherwise). Prior to the labeling, the authors consult together to establish a coding guideline. The second author has a PhD and has published 
peer-reviewed high-impact papers in software security. After that each author 
separately labels the 384 sentences based on the guideline. The agreement analysis is computed between the authors based on two metrics (Cohen Kappa and Percent Agreement). 
The disagreements are resolved by mutual discussions between the authors. For example, there was a disagreement on the following sentence: 
\emt{use a central (admin-type node) SoC/computer on wifi to: \$ curl \$ESP8266\_IP}. After mututal discussions, the 
authors decided to label it as 0 because there is no requirement of security requirements while using the `curl' service from the admin node. 
Finally, the random sample has 17 sentences labeled as security (4.4\%). This is not 
surprising, given that a majority of sentences in IoT posts in forums like SO can have discussions about diverse IoT aspects besides security.    
\item{Judgmental/Opportunistic Sample ($J$).} Given that the the random sample has only 17 sentences labeled as security, the sample 
is not sufficient to provide a comprehensive assemment of the strengths and weakness of SecBot. To pick enough relevant sentences from the IoT posts, we thus 
collect another 600 sentences using a judgmental/opportunistic sampling approach. In judgmental sampling, a random sample of potentially 
relevant items is drawn based on the opinion of an expert~\cite{Marshal-SamplingQualitativeResearch-FamilyPractice1996}. We adopt 
a sampling approach previously used 
to create a benchmark of positive and negative sentences from SO data, where majority of sentences are non-polar~\cite{Calefato-Senti4SD-EMSE2017}. We first run SecBot on all the 
672,678 sentences. We then randomly pick 300 sentences labeled as 1 and another 300 sentences labeled as 0 by SecBot. The intuition is that 
given the high precision of SecBot, the 300 sentences labeled as 1 would probably be precise. We again do manual assessment of the 600 sentences. 
\tbl\ref{tab:validation-sample-stat} shows summary statistics and agreement analysis for the random and jugmental samples. The final validation sample S contains both 
the random and judgment sample (i.e., S = R + J).   
\end{inparaenum} In \tbl\ref{tab:validation-sample-stat}, we show summary statistics of the validation sample. There are total 984 sentences, out of which 32.1\% 
of sentences are labeled as 1 (i.e., they contain security discussions). The last two columns of \tbl\ref{tab:validation-sample-stat} show the agreement 
level between the two coders during their manual labeling. The Cohen kappa value is 0.92 and the percent agreement is 96.7\%. According to 
According to Viera~\cite{Viera-KappaInterpretation-FamilyMed2005}, a kappa value between 0.81 and 0.99 denotes a perfect agreement. 
We run each model trained on API review dataset on the validation sample. We 
analyze whether the performance of the models differs in the validation sample compared their 
performance in the API review dataset. 
\begin{table}[t]
  \centering
  \caption{Summary stats and agreements for the IoT validation sample}
   %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrr|rr}\toprule
    \multirow{2}[0]{*}{\textbf{Sample}} & \multicolumn{3}{c}{\textbf{Summary}} & \multicolumn{2}{c}{\textbf{Agreement}} \\
    \cmidrule{2-6}
          & \textbf{Total Sentences (T)} & \textbf{Sentences Labeled as \#Security (S)} & \textbf{\%S/T} & \textbf{Kappa} & \textbf{Percent} \\
          \midrule
        %IoT Training  & 1000  & 508 &  50.8\%     &   0.97     & 98.5\% \\
        %97.7%	0.744	0.745	0.745
    IoT Validation  & 984   &   316    & 32.1\% & 0.92     &  96.7\%  \\
    
    %95.8%	0.915	0.915	0.915
    
    % \midrule
    % Overall $S$ & 984   &   316    &    33.1\%   & 0.92        & 96.7\% \\
    
    %96.7%	0.917	0.917	0.917
    
    
    \bottomrule
    \end{tabular}%
  %}
  \label{tab:validation-sample-stat}%
\end{table}%
% \begin{table}[t]
%   \centering
%   \caption{Summary stats and agreements for the validation sample}
%   %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{lrrr|rr}\toprule
%     \multirow{2}[0]{*}{\textbf{Sample}} & \multicolumn{3}{c}{\textbf{Summary}} & \multicolumn{2}{c}{\textbf{Agreement}} \\
%     \cmidrule{2-6}
%           & \textbf{Total T} & \textbf{\#Security S} & \textbf{\%S/T} & \textbf{Kappa} & \textbf{Percent} \\
%           \midrule
%         Random $R$ & 384  & 17 &  4.4\%     &   0.75     & 97.7\% \\
%         %97.7%	0.744	0.745	0.745
%     Judgmental $J$ & 600   &   299    & 49.8\% & 0.92     &  95.8\%  \\
    
%     %95.8%	0.915	0.915	0.915
    
%     \midrule
%     Overall $S$ & 984   &   316    &    33.1\%   & 0.92        & 96.7\% \\
    
%     %96.7%	0.917	0.917	0.917
    
    
%     \bottomrule
%     \end{tabular}%
%   %}
%   \label{tab:validation-sample-stat}%
% \end{table}% 
% 
% From RQ2, we found Transformer based RoBERTa model performed better than shallow
% machine learning models and traditinal deep learning models on our security
% related benchmark dataset, $\mathcal{B_{BM}}$. We apply the RoBERTa model
% $\mathcal{M_{BM}}$ on IoT dataset $\mathcal{B}$ to see how the performance
% varies across different security related dataset.\\
% We used nltk sentence tokenizer to segregate sentences from posts of IoT dataset
% $\mathcal{B}$. We got total $672678$ sentences on an average of around $13$
% sentences per post. Then we trained the RoBERTa model $\mathcal{M_{BM}}$ on full
% dataset $\mathcal{B_{BM}}$ using batch size of 16 and run 3 epochs. We labeled
% these $672678$ sentences using this model. Model labeled 8450 sentences as
% security related and rest as non-related. Performance evaluation of our model
% $\mathcal{M}$, on the dataset $\mathcal{B}$, was challenging because we did not
% have either ground truths or the distribution of them which left us nothing but
% choosing the option manual labeling. Without learning the distribution of
% classes, it is difficult to choose any sampling technique or size of the samples
% because if sampled dataset does not generalize the full dataset then performance
% on sampled dataset might equivocate us. A possible solution to this intricacy is
% evaluation of Precision metrics only because Precision depends on instances
% those are only predicted positively by the model. In our experiments, model
% predicted 8450 instances as positive. \textbf{We picked randomly 500,
% approximately 6\%, positively predicted instances. We also picked randomly 500
% (approximately .075\%) instances which are predicted as negative by our model
% $\mathcal{M_{BM}}$.} Because we wanted to infer, model was not missing too many
% positive instances. We merge these 1000 instances to get our new dataset
% $\mathcal{B_{TS}}$. We manually labeled dataset $\mathcal{B_{TS}}$. We reported
% our dataset distribution in Table \ref{tab:datadistribution_confusionmatrix}.\\
% \begin{table}[!h]
%     \centering
%     \begin{tabular}{l|l|c|c|c}
%         \multicolumn{2}{c}{}&\multicolumn{2}{c}{True Label}&\multicolumn{1}{c}{}\\
%         \cline{3-4}
%         \multicolumn{2}{c|}{}&Positive&Negative&\multicolumn{1}{c}{Total}\\
%         \cline{2-4}
%         Prediction by & Positive & $487$ & $13$ & $500$\\
%         \cline{2-4}
%         Model $\mathcal{M_{BM}}$& Negative & $23$ & $477$ & $500$ \\
%         \cline{2-4}
%         \multicolumn{1}{c}{} & \multicolumn{1}{c}{Total} & \multicolumn{1}{c}{$510$} &         \multicolumn{    1}{c}{$490$} & \multicolumn{1}{c}{$1000$} \\
%         
%     \end{tabular}
%     \caption{Dataset Distribution of $\mathcal{B_{TS}}$ and Confusion matrix of Model $\mathcal{M_{BM}}$}
%     \label{tab:datadistribution_confusionmatrix}
% \end{table}

% \begin{figure}[t]%[!htb]
%   \centering
  
%   \includegraphics[scale=.35]{images/pie_chart.pdf}

%   \caption{Class distribution and Performance of $\mathcal{M}$ model on Dataset $\mathcal{B_{TS}}$. Outer circle shows actual distribution of data and inner circle shows prediction of $\mathcal{M_{BM}}$. TP means correctly predicted positives  }

%   \label{fig:pie_chart}

% \end{figure}



% Table generated by Excel2LaTeX from sheet 'Sheet3'
% \begin{table}[t]
%   \centering
%   \caption{SecBot performance on the validation sample (\tbl\ref{tab:validation-sample-stat} \gias{here we show performance of each BERT-based models from RQ2 on te new IoT dataset. We also show how the performance is dropping or increasing from RQ2. We do not break down the performance by random or judgmental sample - simply the entire dataset})}
%     \begin{tabular}{lrrr} \toprule
%     \textbf{Sample Type} & \textbf{P} & \textbf{R} & \textbf{F1} \\ 
%     \midrule
%     On Random Sample (R) & 0.75  & 0.19  & 0.30 \\
%     On Judgmental Sample (J) & 0.72  & 0.70  & 0.71 \\
%     \midrule
%     On Overall Validation Sample (S) & 0.72  & 0.68  & 0.70 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:performance-secbot-valsample}%
% \end{table}%
% \begin{table}
% \centering
%    \caption{Performance of various Transformer models on IoT Validation}
%  \begin{tabular}{l|rrrrr} 
%  \toprule
%  \bf{Model} & \bf{P} & \bf{R} & \bf{F1} & \bf{AUC} & \bf{MCC}\\  
%  \midrule
%  BERT &0.794 &	0.683 &	0.735 &	0.8 &	0.626\\
%  RoBERTa & 0.957 &	0.633 &	0.762 &	0.81 &	0.707 \\ 
%  DistilBERT & 0.945 &	0.553 &	0.698 &	0.769 &	0.643 \\
%  ALBERT & 0.989 &	0.598 &	0.745 &	0.798 &	0.703 \\
%  XLNet & 0.901 &	0.607 &	0.726 &	0.788 &	0.653\\
%  \midrule
%  Baseline-SVM & 0.981 &	0.326 &	0.489 &	0.661 &	0.488\\
%  Baseline-Logits & 0.98 &	0.32 &	0.482 &	0.658 &	0.483\\
%  LSTM & 0.93 &	0.59 &	0.725 &	0.787 &	0.663\\
%  Bi-LSTM & 0.858 &	0.613 &	0.715 &	0.783 &	0.628\\
%  \midrule
% \multicolumn{6}{c}{Performance change (\%) in RoBERTa over Baseline and Traditional Deep Models}\\
%  \midrule
%  Baseline-Logits & 2.4\%$\downarrow$ & 94.2\%$\uparrow$ & 55.8\%$\uparrow$ & 22.5\%$\uparrow$ & 44.9\%$\uparrow$ \\
%  Baseline-SVM & 2.3\%$\downarrow$ & 97.8\%$\uparrow$ & 58.1\%$\uparrow$ & 23.1\%$\uparrow$ & 46.4\%$\uparrow$\\
%  LSTM &  2.9\%$\uparrow$ &  7.3\%$\uparrow$ & 5.1\%$\uparrow$ & 2.9\%$\uparrow$ & 6.6\%$\uparrow$\\
%  Bi-LSTM & 11.5\%$\uparrow$ & 3.3\%$\uparrow$ & 6.6\%$\uparrow$ & 3.4\%$\uparrow$ & 12.6\%$\uparrow$\\
%  \bottomrule
%  \bottomrule
% \end{tabular}
%     \label{tab:bert_performance}
% \end{table}

% Table generated by Excel2LaTeX from sheet 'RQ2'
\begin{table}[htbp]
  \centering
  \caption{Performance of Models Trained Using API Review Dataset on IoT Validation Sample}
    \begin{tabular}{llrrrrr}\toprule
    \multicolumn{1}{l}{\textbf{Model Type}} & \textbf{Model Name} & {\textbf{P}} & {\textbf{R}} & {\textbf{F1}} & {\textbf{Acc}} & {\textbf{AUC}} \\
    \midrule
    {Baseline Shallow} & SVM   & 0.981 & 0.326 & 0.489 & 0.782 & 0.661 \\
          & \%Change from API Review Dataset & 43.4\%\up & -57.1\%\dn & -31.4\%\dn & -20.0\%\dn & -24.3\%\dn \\
          \cmidrule{2-7}
          & Logit & 0.98  & 0.32  & 0.482 & 0.78  & 0.658 \\
          & \%Change from API Review Dataset & 43.7\%\up & -59.8\%\dn & -33.8\%\dn & -20.2\%\dn & -26.2\%\dn \\
          \midrule
    {seq2seq} & LSTM  & 0.878 & 0.503 & 0.64  & 0.818 & 0.735 \\
          & \%Change from API Review Dataset & 24.9\%\up & -28.1\%\dn & -8.3\%\dn & -16.3\%\dn & -12.9\%\dn \\
          \cmidrule{2-7}
          & Bi-LSTM & 0.764 & 0.585 & 0.663 & 0.815 & 0.75 \\
          & \%Change from API Review Dataset & 5.8\%\up & 0.5\%\up & 5.2\%\up & -16.5\%\dn & -4.6\%\dn \\
          \midrule
    {Transformer} & BERT  & 0.794 & 0.683 & 0.735 & 0.841 & 0.735 \\
          & \%Change from API Review Dataset & 10.0\%\up & -15.5\%\dn & 0.3\%\up & -14.3\%\dn & -18.0\%\dn \\
          \cmidrule{2-7}
          & \bf{SecBot} (RoBERTa) & 0.957 & 0.633 & \textbf{0.762} & 0.873 & 0.81 \\
          & \%Change from API Review Dataset & 29.0\%\up & -27.3\%\dn & \bf{-4.0\%\dn} & -11.3\%\dn & -12.8\%\dn \\
          \cmidrule{2-7}
          & XLNet & 0.901 & 0.607 & 0.726 & 0.852 & 0.788 \\
          & \%Change from API Review Dataset & 31.3\%\up & -25.0\%\dn & -0.3\%\dn & -13.0\%\dn & -12.1\%\dn \\
          \cmidrule{2-7}
          & ALBERT & 0.989 & 0.598 & 0.745 & 0.869 & 0.798 \\
          & \%Change from API Review Dataset & 27.6\%\up & -17.4\%\dn & 1.1\%\up & -11.5\%\dn & -6.9\%\dn \\
          \cmidrule{2-7}
          & DistilBERT & 0.945 & 0.553 & 0.698 & 0.846 & 0.769 \\
          & \%Change from API Review Dataset & 23.7\%\up & -27.2\%\dn & -4.0\%\dn & -13.8\%\dn & -12.0\%\dn \\
          \bottomrule
    \end{tabular}%
  \label{tab:performanceCrossDataset}%
\end{table}%

\begin{figure}[t]%[!htb]
  \centering
  \includegraphics[scale=.55]{images/SecBot_ROC.pdf}

  \caption{ROC curve for SecBot (i.e., RoBERTa trained on API review dataset) model on the validation sample}

  \label{fig:roc-roberta}

\end{figure}
\subsubsection{Results} We present the performance of models trained using Opiner API review dataset on our newly created IoT 
validation sample in \tbl\ref{tab:performanceCrossDataset}. Similar to the API review dataset, 
SecBot (i.e., the trained RoBERTa model) remains the best performing classifier in the validation sample with an F1-score of 0.762. However, 
compared the the API review dataset, the F1-score of SecBot in the validation sample has decreased by 4\%. This means that 
while SecBot does not suffer from large drop in performance, there are still some new instances/ways of expressing sentiment discussions in IoT 
validation sample compared to the API review dataset. Not all the models, however, show a drop in performance in terms of F1-score. For example, 
three models (BERT, ALBERT, and Bi-LSTM) shows better F1-score in the validation sample than they show in the API review dataset. However, 
such slight increase is mainly due to the higher precisions the models show in the IoT sample, while all the models show very low recall compared 
to the API review dataset. This means that the models miss a considerable number of true positives in IoT sample, but when they detect a sentence as 
containing security discussions they are mostly correct. This observation can further be explained by analyzing the ROC curvey of SecBot. In \fig\ref{fig:roc-roberta}, 
we show the ROC curve of SecBot on the IoT validation sample. The model shows a high F1-score of at least 0.8 with a threshold (of TPR/TFR ratio) 0.4. 
This denotes that the model is confident of positive cases when it sees one based on what it saw in the API review dataset. However, this 
rapid upswing also denotes that the model is also confident to discard positive cases that it has not seen before. Therefore, 
the models can benefit from a re-training based on both the API review dataset and sentences from our IoT dataset of 53K posts.
 
% SecBot shows an F1-score of 0.70 on the entire validation sample. This means that the performance of SecBot 
% has dropped slightly from its F1-score of 0.80 on Opiner benchmark (\sec\ref{sec:detect-security-aspect}). This is not 
% surprising given that the Opiner benchmark does not have any IoT discussions. The drop in performance is mainly due to the 
% drop in recall (0.68 in the validation sample vs 0.83 in Opiner benchmark) and not much in precision (0.72 in the validation sample 
% vs 0.77 in the Opiner benchmark). This means that SecBot is missing positive cases in the validation sample because of the specificity of security 
% discussions in IoT sample. Overall, the drop in SecBot performance in the validation sample is mainly due to its low 
% performance in the Random sample (R) dataset, where it shows an F1-score of 0.30. For this sample, SecBot shows a precision of 0.75 which is better than its 
% precision of 0.72 in the judgmental sample. However, the SecBot shows a recall of only 0.19 in random sample. This is because SecBot 
% was able to correctly label only 4 out of the 17 positive cases in the random sample. For example, SecBot could not detect that the following 
% sentence refers to the security in an IoT hub: \emt{The device is not behind firewall or any special network topology used, it connects to the IoT Hub via MQTT.} The reason 
% is that such positive cases are not found in the Opiner benchmark, hence SecBot had no previous knowledge of those. Therefore, the performance of SecBot 
% can be improved on our validation sample, if the RoBERTa model in SecBot can be retrained using IoT discussions in addition to the data from Opiner benchmark. 
%In RQ4, we aim to improve the performance of SecBot for IoT discussions.   

%\gias{Can we create a statistically significant sample of the misclassified sentences by the best performing BERT-model here? We will then label each sentence to determine the reason of misclassification, e.g., lack of contextual info, general error, etc. See Figure 12 and Misclassification Analysis of my paper on how to do that \url{https://giasuddin.files.wordpress.com/2020/12/tse2019b-automaticminingofopinionsfromso.pdf} (Pages 28, 29)}
%\gias{once the above table is created, explain it the way I explained it in my paper.}
% \subsubsection{\textbf{Results}}
% In Table \ref{tab:datadistribution_confusionmatrix}, we showed dataset distribution along with prediction of model $\mathcal{B_{TS}}$ on that dataset. Dataset $\mathcal{B_{TS}}$ contains 510(51\%) positive instances and 490(49\%) negative instances. \textbf{Out of 500 positive predictions made by model $\mathcal{M}$, 487 are correct and 13 are incorrect which indicates, model is predicting precisely with a massive Precision of .974 which is approximately 50\% better than previous performance on dataset $\mathcal{B_{BM}}$}. We also compared this metrics with previously evaluated metrics on dataset $\mathcal{B_{BM}}$, shown in Table \ref{tab:performance_on_BM_TS}. Model performance on this dataset is more precise and accurate than on dataset $\mathcal{B_{BM}}$. High recall suggests, model is exploring almost all positive instances present in dataset. But from this we could not infer that model would explore all security related sentences if it tested on dataset $\mathcal{B}$. Because we did not know the actual distribution of the dataset and also we chose almost a balanced dataset. We could not fully rely on Recall and so we mostly focused on Precision in evaluation our model.\\
% \begin{table}[!h]
%     \begin{center}
%  \begin{tabular}{c|ccccc} 
%  \hline\hline
%  Dataset & &P && R & F1 \\ [0.5ex] 
%  \hline
%  $\mathcal{B_{TS}}$ && .97 && .95 & .96 \\
%  $\mathcal{B_{BM}}$ & &.77 && .83 & .8 \\
%  \hline
%  \multicolumn{6}{c}{Performance increase(\%) on dataset $\mathcal{B_{TS}}$ over dataset$\mathcal{B_{BM}}$}\\
%  \hline
%  \multicolumn{1}{c}{}&& 25.97\% && 14.58\%& 20.0\%\\
%  \hline\hline
% \end{tabular}
% \end{center}
% 
% 
% 
%     \caption{Performance of RoBERTa model $\mathcal{M_{BM}}$ on dataset $\mathcal{B_{TS}}$ and $\mathcal{B_{BM}}$ }
%     \label{tab:performance_on_BM_TS}
% \end{table}
% High Precision surely indicates our success in the experiment. This high Precision is because of dataset domain. Dataset $\mathcal{B_{BM}}$ was created from various Stack Overflow post related to programming where security related tags, cryptography and authentication were included. `Signed key', `private token', `unwanted', `access permission', etc are commonly used in those sentences and model underlines these words during prediction. As a result model fails to distinguish between these words and programming related words `Signed bit', `unsigned bit', `unwanted variable', `unwanted errors', `access modifier', `private variable' etc. On the contrary, dataset $\mathcal{B}$ were collected from various tags related to IoT and security one of the key aspects of IoT that is why our model performed better on this dataset.\\




% Table generated by Excel2LaTeX from sheet 'Sheet2'
% \begin{table}[t]
%   \centering
%   \caption{Summary stats and agreements on IoT training sample \gias{This table is no longer required}}
%     \begin{tabular}{rrrr|rr}\toprule
%     \multicolumn{4}{c}{\textbf{Summary}}  & \multicolumn{2}{c}{\textbf{Agreement}} \\
%     \midrule
%     {\textbf{Total T}} & {\textbf{\#Security S}} & {\textbf{\%S/T}} & {\textbf{Non-Security}} & {\textbf{Kappa}} & {\textbf{Percent}} \\
%     \midrule
%     1,000  & 508   & 50.8\% & 492   & 0.97      & 98.5\% \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:iot-training-sample}%
% \end{table}%



% \begin{table}
% \centering
%   \caption{Performance of various Transformer models}
%  \begin{tabular}{l|rrrr} 
%  \toprule
%  \bf{Model} & \bf{P} & \bf{R} & \bf{F1} \\  
%  \midrule
%  BERT & 0.927 & 0.848 & 0.886\\
%  XLNet & 0.958 & 0.78 & 0.86\\ 
%  DistilBERT & 0.936 & 0.781 & 0.852\\
%  ALBERT & 0.99 & 0.812 & 0.892\\
%  FunnelBERT & 0.975 & 0.715 & 0.825\\
%  ELECTRA & 0.989 & 0.75 & 0.853\\
%  RoBERTa & 0.885 & 0.905 & 0.895\\
%  SVM & 0.989 & 0.351 & 0.518\\
%  Logits & 0.989 & 0.348 & 0.515\\
%  \midrule
%  \bottomrule
% \end{tabular}
%     \label{tab:bert_performance}
% \end{table}


\subsection{Improvement of the Models By Adding Sentences from IoT Dicussions in Training (RQ3)}\label{sec:rq-secbotplus-dev}
The results from RQ2 show that the models trained on API review dataset exhibit a drop in performance in the IoT validation dataset. 
We, therefore, aim to improve the performance of the models by preparing a benchmark of IoT sentences from our 53K IoT posts. 
%We then 
%retraining the models based on a combined dataset of API review and the IoT benchmark. 
%We prepare a training sample from our IoT posts and use it  to retrain the RoBERTa model that we used for SecBot. 
\subsubsection{Approach} We prepare the training sample of 1,000 sentences by following the same approach we used to create the judgmental sample in 
\sec\ref{sec:rq-secbot-assess-iot}. This is because, as we observed in \sec\ref{sec:rq-secbot-assess-iot}, a random sampling would produce a very skewed dataset with 
low number of sentences with discussions about security. Indeed, judgmental sampling is used to create training sample from such imbalanced real-world datsets ~\cite{Calefato-Senti4SD-EMSE2017,Socher-Sentiment-EMNLP2013}. 
We created the training sample as follows. First, we randomly pick 500 sentences labeled as 1 and another 500 sentences labeled as 0 
by SecBot from the 672,678 of the 53K IoT posts. To ensure fair comparison between 
SecBot and the new model. The 1,000 new sentences do not have any overlap with the 
984 sentences in our validation sample in \tbl\ref{tab:validation-sample-stat}. Second, we manually labeled each sentence. The first two authors worked together 
to do the manual labeling by following a shared understanding process previously used in literature~\cite{Kononenko-CodeReviewQuality-ICSE2016,Uddin-OpinionValue-TSE2019}. The 
process works as follows. Both of the authors separately labeled the same 200 sentences out of the training sample, 
100 from each case (i.e, 1 and 0). The agreements between the 
authors is computed using Cohen Kappa and Percent Agreement. The Kappa agreement was more than 0.90, i.e, the two authors reached a perfect agreement. 
Therefore, after this round, any of the authors can finish the rest of the labels without introducing subjective bias. This is not 
surprising given that the two authors have manually labeled the entire validation sample before. After this, the first author completed the rest of the 
labels. \tbl\ref{tab:iot-training-sample-stat} shows summary statistics of the training sample and the agreement analysis between the authors. Out of the 1,000 
sentences, 508 sentences are labeled as 1 (i.e., contains security discussion). Third, we combine the 1,000 sentences with the 4,297 sentences from Opiner benchmark. 
The combined training dataset has  5,297 labeled sentences, out of which 671 sentences are labeled as 1 (ratio = 12.7\%). We use this combined dataset to 
retrain the models we studied in this paper. While 1000 new sentences may seem insufficient for deep learning models, we previously found that 
pre-trained advanced lanaguage models (i.e, the transformer) models often offer good performance with little data due to the fact that the models are already 
pre-trained on large sample cross-domain data~\cite{Khan-FakeNews-MLWA2021}. %(i.e., SVM and Logit).
% - the same models that 
%we previously we used to train SecBot on Opiner benchmark. We call the new model \bf{\ul{SecBot+}}.

% \begin{table}[t]
% \centering
% \caption{Hyperparameters of BERT variants}
% \begin{tabular}{l|c|c|rrr}
% \toprule
% \textbf{Model}& \bf{Optimizer} & \bf{Loss Functions} & \bf{Batch Size} & \bf{Epochs}   & \bf{Learning Rate}\\ 
% \midrule
%  BERT & \multirow{5}[0]{*}{Adam} & \multirow{5}[0]{*}{binary-crossentropy} & 32 & 3 & 3e-5\\ 
%  RoBERTa &   &&32 & 2 & 1e-5\\
%  XLNet &  &&32 & 3  & 1e-5\\
%  ALBERT &  &&32 & 3  & 1e-5\\
%  DistilBERT &&&  32 & 3 & 1e-5\\
%  %FunnelBERT & funnel-transformer/small-base &12& 768 & 12 & 115M \\
%  %ELECTRA& google/electra-small-discriminator&  12&	256&12 &	14M\\
% \bottomrule
% \end{tabular}
% %}
% \label{BERT Hyperparameters} 
% %\end{center}
% \end{table}
\begin{table}[t]
  \centering
  \caption{Summary stats and agreements for the IoT training dataset}
   %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{lrrr|rr}\toprule
    \multirow{2}[0]{*}{\textbf{Sample}} & \multicolumn{3}{c}{\textbf{Summary}} & \multicolumn{2}{c}{\textbf{Agreement}} \\
    \cmidrule{2-6}
          & \textbf{Total Sentences (T)} & \textbf{Sentences Labeled as \#Security (S)} & \textbf{\%S/T} & \textbf{Kappa} & \textbf{Percent} \\
          \midrule
        IoT Training  & 1000  & 508 &  50.8\%     &   0.97     & 98.5\% \\
        %97.7%	0.744	0.745	0.745
    %IoT Validation  & 984   &   316    & 33.1\% & 0.92     &  96.7\%  \\
    
    %95.8%	0.915	0.915	0.915
    
    % \midrule
    % Overall $S$ & 984   &   316    &    33.1\%   & 0.92        & 96.7\% \\
    
    %96.7%	0.917	0.917	0.917
    
    
    \bottomrule
    \end{tabular}%
  %}
  \label{tab:iot-training-sample-stat}%
\end{table}%
\begin{table}[t]
\centering
\caption{Hyperparameters of the deep learning models on the Combined dataset (API review + IoT Benchmark)}
\begin{tabular}{p{2cm}l|rrrrr}
\toprule
\bf{Type} & \textbf{Model}& \bf{Batch Size} & \bf{Epochs}  & \bf{Optimizer} & \bf{Loss Functions} & \bf{Learning Rate}\\ 
\midrule
\multirow{2}[0]{*}{Seq2Seq} &  LSTM & 64 & 50 & Adam & binary-crossentropy & 2e-3\\ 
& Bi-LSTM & 64 & 20 & Adam & binary-crossentropy & 2e-3\\
 \midrule
\multirow{5}[0]{*}{Transformer} & BERT & 32 & 3 & Adam & binary-crossentropy & 3e-5 \\
& RoBERTa & 32 & 3 & Adam & binary-crossentropy & 1e-5 \\
& XLNet & 32 & 2 & Adam & binary-crossentropy & 1e-5 \\
& ALBERT & 32 & 3 & Adam & binary-crossentropy & 1e-5 \\
& DistilBERT & 32 & 3 & Adam & binary-crossentropy & 1e-5\\
 %FunnelBERT & funnel-transformer/small-base &12& 768 & 12 & 115M \\
 %ELECTRA& google/electra-small-discriminator&  12&	256&12 &	14M\\
\bottomrule
\end{tabular}
%}
\label{dllParamCombined} 
%\end{center}
\end{table}


% \begin{table}
% \centering
%    \caption{Cross validation performance of Transformers on Opiner + IoT training samples}
%  \begin{tabular}{l|rrrrr} 
%  \toprule
%  \bf{Model} & \bf{P} & \bf{R} & \bf{F1} & \bf{AUC} & \bf{MCC}\\  
%  \midrule
%  BERT &0.92&	0.904 & 0.91 & 0.946 &	0.898\\
%  RoBERTa & 0.888 & 0.939 & 0.912 & 0.961 & 0.9 \\ 
%  DistilBERT & 0.89 & 0.911 & 0.901 & 0.947 & 0.888 \\
%  ALBERT & 0.91	& 0.885& 0.897& 0.936 & 0.883 \\
%  XLNet & 0.871 & 0.929 & 0.898 & 0.954 & 0.884\\
%  \midrule
%  Baseline-SVM & 0.812 & 0.89 & 0.848 & 0.93 & 0.828\\
%  Baseline-Logits & 0.801 & 0.891 &	0.843 &	0.93 &	0.822\\
%  LSTM & 0.866 & 0.861 & 0.861 &	0.92 &	0.842\\
%  Bi-LSTM & 0.861 & 0.849 & 0.854 & 0.914& 0.833\\
%  \midrule
% \multicolumn{6}{c}{Performance change (\%) in RoBERTa over Baseline and Traditional Deep Models}\\
%  \midrule
%  Baseline-Logits & 9.4\%$\downarrow$ & 5.5\%$\uparrow$ & 7.5\%$\uparrow$ & 3.3\%$\uparrow$ & 8.7\%$\uparrow$ \\
%  Baseline-SVM & 10.9\%$\downarrow$ & 5.4\%$\uparrow$ & 8.2\%$\uparrow$ & 3.3\%$\uparrow$ & 9.5\%$\uparrow$\\
%  LSTM &  2.5\%$\uparrow$ &  9.1\%$\uparrow$ & 5.9\%$\uparrow$ & 4.5\%$\uparrow$ & 6.9\%$\uparrow$\\
%  Bi-LSTM & 3.1\%$\uparrow$ & 10.6\%$\uparrow$ & 6.8\%$\uparrow$ & 5.1\%$\uparrow$ & 8.0\%$\uparrow$\\
%  \bottomrule
%  \bottomrule
% \end{tabular}
%     \label{tab:bert_performance}
% \end{table}
% 
% \begin{table}
% \centering
%    \caption{Performance of Transformers on IoT validation samples}
%  \begin{tabular}{l|rrrrr} 
%  \toprule
%  \bf{Model} & \bf{P} & \bf{R} & \bf{F1} & \bf{AUC} & \bf{MCC}\\  
%  \midrule
%  BERT &0.886 &	0.787 &	0.834 &	0.87 &	0.765\\
%  RoBERTa & 0.9 &	0.877 &	0.888 &	0.915 &	0.836 \\ 
%  DistilBERT & 0.864	& 0.784 &	0.822 &	0.863 &	0.746 \\
%  ALBERT & 0.891	& 0.803 &	0.845 &	0.878 &	0.78 \\
%  XLNet & 0.868	& 0.769 &	0.815 &	0.857 &	0.738\\
%  \midrule
%  Baseline-SVM & 0.748 &	0.753 &	0.751 &	0.817 &	0.632\\
%  Baseline-Logits & 0.735 &	0.753 &	0.744 &	0.812 &	0.62\\
%  LSTM & 0.826 &	0.782	& 0.803 &	0.852 &	0.714\\
%  Bi-LSTM & 0.753 &	0.822 &	0.787 &	0.848 &	0.681\\
%  \midrule
% \multicolumn{6}{c}{Performance change (\%) in RoBERTa over Baseline and Traditional Deep Models}\\
%  \midrule
%  Baseline-Logits & 20.3\%$\downarrow$ & 16.5\%$\uparrow$ & 18.2\%$\uparrow$ & 12.0\%$\uparrow$ & 32.3\%$\uparrow$ \\
%  Baseline-SVM & 22.4\%$\downarrow$ & 16.5\%$\uparrow$ & 19.4\%$\uparrow$ & 23.0\%$\uparrow$ & 34.9\%$\uparrow$\\
%  LSTM &  0.2\%$\uparrow$ &  12.1\%$\uparrow$ & 10.6\%$\uparrow$ & 7.4\%$\uparrow$ & 17.1\%$\uparrow$\\
%  Bi-LSTM & 19.5\%$\uparrow$ & 6.7\%$\uparrow$ & 12.8\%$\uparrow$ & 7.9\%$\uparrow$ & 22.8\%$\uparrow$\\
%  \bottomrule
%  \bottomrule
% \end{tabular}
%     \label{tab:bert_performance}
% \end{table}

% Table generated by Excel2LaTeX from sheet 'RQ3'
\begin{table}[t]
  \centering
  \caption{Performance of the models (trained using combined dataset) on the IoT validation sample}
    \begin{tabular}{rlrrrrr}\toprule
    \multicolumn{1}{l}{\textbf{Model Type}} & \textbf{Model Name} & {\textbf{P}} & {\textbf{R}} & {\textbf{F1}} & {\textbf{Acc}} & {\textbf{AUC}} \\
    \midrule
    \multicolumn{1}{l}{Baseline} & SVM   & 0.748 & 0.753 & 0.751 & 0.839 & 0.817 \\
          & \%Change from Trained Using API Review Dataset & -23.8\%\dn & 131.0\%\up & 53.6\%\up & 7.3\%\up & 23.6\%\up \\
          \cmidrule{2-7}
          & Logit & 0.735 & 0.753 & 0.744 & 0.833 & 0.812 \\
          & \%Change from Trained Using API Review Dataset & -25.0\%\dn & 135.3\%\up & 54.4\%\up & 6.8\%\up & 23.4\%\up \\
          \midrule
    \multicolumn{1}{l}{Seq2Seq} & LSTM  & 0.826 & 0.782 & 0.803 & 0.877 & 0.852 \\
          & \%Change from Trained Using API Review Dataset & -5.9\%\dn & 55.5\%\up & 25.5\%\up & 7.2\%\up & 15.9\%\up \\
          \cmidrule{2-7}
          & Bi-LSTM & 0.753 & 0.822 & 0.787 & 0.856 & 0.848 \\
          & \%Change from Trained Using API Review Dataset & -1.4\%\dn & 40.5\%\up & 18.7\%\up & 5.0\%\up & 13.1\%\up \\
          \midrule
    \multicolumn{1}{l}{Transformer} & BERT  & 0.886 & 0.787 & 0.834 & 0.899 & 0.87 \\
          & \%Change from Trained Using API Review Dataset & 11.6\%\up & 15.2\%\up & 13.5\%\up & 6.9\%\up & 18.4\%\up \\
          \cmidrule{2-7}
          & \bf{SecBot+ (RoBERTa)} & 0.9   & 0.877 & \bf{0.888} & 0.929 & 0.915 \\
          & \%Change from Trained Using API Review Dataset & -6.0\%\dn & 38.5\%\up & \bf{16.5\%\up} & 6.4\%\up & 13.0\%\up \\
          \cmidrule{2-7}
          & XLNet & 0.868 & 0.769 & 0.815 & 0.888 & 0.857 \\
          & \%Change from Trained Using API Review Dataset & -3.7\%\dn & 26.7\%\up & 12.3\%\up & 4.2\%\up & 8.8\%\up \\
          \cmidrule{2-7}
          & ALBERT & 0.891 & 0.803 & 0.845 & 0.905 & 0.878 \\
          & \%Change from Trained Using API Review Dataset & -9.9\%\dn & 34.3\%\up & 13.4\%\up & 4.1\%\up & 10.0\%\up \\
          \cmidrule{2-7}
          & DistilBERT & 0.864 & 0.784 & 0.822 & 0.891 & 0.863 \\
          & \%Change from Trained Using API Review Dataset & -8.6\%\dn & 41.8\%\up & 17.8\%\up & 5.3\%\up & 12.2\%\up \\
          \bottomrule
    \end{tabular}%
  \label{tab:performance-secbotplus-valsample}%
\end{table}%
\begin{figure}[t]%[!htb]
  \centering
  \includegraphics[scale=.55]{images/SecBot+_ROC.pdf}

  \caption{ROC curve for SecBot+ (i.e., RoBERTa trained on combined dataset) model on the validation sample}

  \label{fig:roc-roberta}

\end{figure}


% Table generated by Excel2LaTeX from sheet 'Sheet4'
% \begin{table}[t]
%   \centering
%   \caption{SecBot+ performance on validation sample (\tbl\ref{tab:validation-sample-stat})\gias{here we show the performance of all BERT models on the IoT-only and the combined dataset. }}
%     \begin{tabular}{llrrr}\toprule
%     \textbf{Sample} & \textbf{Model} & \textbf{P} & \textbf{R} & \textbf{F1} \\
%     \midrule
%     \multirow{2}[0]{*}{Overall} & SecBot+ & 0.92  & 0.93  & 0.92 \\
%           & \% Improve over SecBot & 27.8\%$\uparrow$ & 36.8\%$\uparrow$ & 31.4\%$\uparrow$ \\
%           \midrule
%     \multirow{2}[0]{*}{Random} & SecBot+ & 0.85  & 0.65  & 0.73 \\
%           & \% Improve over SecBot & 13.3\%$\uparrow$ & 242.1\%$\uparrow$ & 143.3\%$\uparrow$ \\
%           \midrule
%     \multirow{2}[0]{*}{Judgmental} & SecBot+ & 0.93  & 0.91  & 0.92 \\
%           & \% Improve over SecBot & 29.2\%$\uparrow$ & 30.0\%$\uparrow$ & 29.6\%$\uparrow$ \\
%           \bottomrule
%     \end{tabular}%
%   \label{tab:performance-secbotplus-valsample}%
% \end{table}%
\subsubsection{Results} Similar to the hyperparameter tuning process we applied during our analysis of API review dataset (i.e., RQ1), we conduct 
a Grid search for each studied model to determine their hyperparameter in our combined benchmark. In \tbl\ref{dllParamCombined}, we show 
selected hyperparameters and their values after tuning. We train each model using the combined dataset. We then compute the performance 
of each model on the IoT validation sample. In \tbl\ref{tab:performance-secbotplus-valsample}, we show the performance of the baseline shallow 
learning models from Opiner (i.e., SVM and Logit) and the studied deep learning models on the validation sample. 

Similar to the API review dataset, the RoBERTa-based model showed the best F1-score (0.888) out of all the models on the combined 
dataset. We call the new model \bf{\ul{SecBot+}} for future reference. SecBot+ shows an increase of 16.5\% in F1-score over SecBot on the IoT validation 
sample. Therefore, the inclusion of IoT-specific sentences into the training has contributed to the increase of performance in the models. The increase 
in performance is also prominent in the 38.5\% increase in recall of SecBot+ over SecBot. However, compared to SecBot, SecBot+ shows a slight decrease in 
precision (6\% drop). This means that SecBot+ is more robust in terms of detecting security aspect in the combined dataset, but due to this expanded reach 
SecBot+ can also sometimes be a bit less precise than SecBot. Overall, the increase in performance in SecBot+ compared to SecBot can be shown through an ROC 
curve of SecBot+ in the IoT validation sample (see \fig\ref{fig:roc-roberta}). As we see in \fig\ref{fig:roc-roberta}, SecBot+ reaches an F1-score of at least 0.8 within a 
threshold of 0.2 compared to 0.4 for SecBot. For example, SecBot+ corrected the following 
misclassification of SecBot with right label of 1: \emt{For distribution of the private key after manufacture, it gets a bit more complicated because you're effectively creating another channel for devices to be managed in your registry.}. 
SecBot+ was able to do that because the new 1,000 IoT-related sentences in the combined benchmark offered information about authentication (using private key) 
over IoT communication channels. Similarly, the following misclassification by SecBot in the random sample that we shown in \sec\ref{sec:rq-secbot-assess-iot} was also 
corrected by SecBot+: \emt{The device is not behind firewall or any special network topology used, it connects to the IoT Hub via MQTT.}    

Overall, all the models we have studied show an increase in their performance (based on F1-score) on the validation sample, once the models are trained using the combined 
sample (see \tbl\ref{tab:performance-secbotplus-valsample}). Therefore, the introduction of IoT-related 
discussions into the Opiner benchmark offered a more precise detector for IoT security discussions. SecBot+ can be used to detect and analyze 
IoT security-related discussions with reasonable confidence. 



%\gias{now can we show how many of the previously misclassified categories are corrected here?}
% \subsubsection{\textbf{Approach}}
% Our success on dataset $\mathcal{B_{TS}}$, created opportunity to explore more about Model $\mathcal{M}$. We already discussed that model $\mathcal{M_{BM}}$ was trained on small dataset which had particularly cryptography and authentication related sentences from security domain. So, we could not expect model to perform well uniformly on all others domain. Model requires to be trained on various types of security related topics so that it can learn about those fields and predict more confidently and accurately. We took advantages of dataset $\mathcal{B_{TS}}$ which was labeled manually, discussed in \ref{RQ3_approach}. Although out of the 510 positives 487 are correctly predicted by model $\mathcal{M}$, rest 23 data can help model to get more insight about security and of course, compared to 163 instaces in dataset $D_{BM}$, 510 more instances will surely give the model more insights and confidence as well. For example, assume dataset contains key related only two sentences, ``You can not change primary key as it is auto generated" and ``You can not change key as it is your identity" labeled as 0 and 1 respectively. Now for any model, it is almost impossible to learn the context of the word ``key" from this two sentences only. Now, if we add more sentences with word ``key" then model might understand the context.\\
% \textbf{We merged our two dataset $\mathcal{B_{BM}}$ and $\mathcal{B_{TS}}$ to get new dataset $\mathcal{B_{MS}}$ with 673 positive instances.} Then, Pretrained RoBERTa, discuss in \ref{RQ2_approach}, was trained on this merged dataset $\mathcal{B_{MS}}$ using $10-fold~cross~validation$, discussed in \ref{RQ1_approach}. Later, this model was trained on full dataset $\mathcal{B_{MS}}$ to get our new model $\mathcal{M_{MS}}$. We called this model as $\mathcal{M_{MS}} $. Our next challenge was, how to evaluate performance of these models and compare between them as well. Both model have same architecture, parameters and even identical hyperparameters. Seemingly, The only difference is dataset that is feed into them. From previous experiments results, it can easily be showed that more that 99\% data of dataset $\mathcal{B_{MS}}$ are achievable by model $\mathcal{M}$. In addition to this, ratio of the positive instances increases by more than 200\% which implies that more positive instances is present in validation set and also most of these validation data are from dataset $\mathcal{B_{TS}}$ which can be classified with high Precision by model $\mathcal{M}$. So, we can say both dataset are almost identical which raises the questions, are the model exploring whole security domain or just cryptography, and authentication? So there are enough doubts that can not be answered only by showing good performance on $10-fold~cross~validation$. We answer those questions using different approaches.\\
% We labeled our full dataset using model $\mathcal{M_{MS}}$. Model reported 30192 instances as positive and rest as negative. We reported prediction of this model along with the prediction of model $\mathcal{M}$ in Figure \ref{fig:agreement_matrix}. \textbf{Figure \ref{fig:agreement_matrix} shows both models agree in 96.71\% sentences where they disagree in 3.29\% sentences.} $\mathcal{M_{MS}}$ found more that 250\% positive instances which needed to be verified either this model predicted them correctly or not. These stats showed model $\mathcal{M_{MS}}$ might be more effective in exploring positive instances than model $\mathcal{M}$ but of course, first we needed human level validation on those instances. \textbf{That is why we created a dataset $\mathcal{B_{DS}}$ picking 200 instances, 100 randomly from .03\% disagreement instances and others randomly from rest 3.26\% disagreement instances. To answer all the questions stated earlier, we created two more datasets. Dataset $\mathcal{B_{AS}}$ was created from random 100 instances from 1.22\% agreements and 100 from 95.49\%. For final dataset $\mathcal{B_{BS}}$, we picked 100 random instances of each type which were labeled as positive and negative by model $\mathcal{M}$.} Then we manually labeled all these three datasets and evaluated Precision, Recall, F1-Score of both models.\\    
% 
% \begin{figure}[!h]%[!htb]
%   \centering
%   \includegraphics[scale=.7]{images/agreement_matrix.pdf}
% 
%   \caption{Agreement and Disagreement of model $\mathcal{M}$ and model $\mathcal{M_{MS}}$ on dataset $\mathcal{B}$}
% 
%   \label{fig:agreement_matrix}
% 
% \end{figure}
% 
% 
% \begin{table}[!h]
%     \begin{center}
%  \begin{tabular}{c| c c c c} 
%  \hline
%  Dataset & Model & P & R & F1\\ 
%  \hline
%  $\mathcal{B_{BM}}$&$\mathcal{M}$ & .77 & .83 & .80\\  
%  $\mathcal{B_{BM} }$ \& $\mathcal{B_{TS}}$ &$\mathcal{M_{MS}}$ & .90 & .93 & .91 \\
%  \hline
%  \multicolumn{5}{c}{Performance increase(\%) of model $\mathcal{M_{MS}}$ over $\mathcal{M}$}\\
%  \hline
%  \multicolumn{2}{c}{}& 16.88\% & 12.05\%& 13.75\%\\
%  \hline\hline
% \end{tabular}
% \end{center}
% 
% 
% 
%     \caption{Performance of $\mathcal{M}$ and $\mathcal{M}$ models}
%     \label{tab:comparison_M vs M_MS}
% \end{table}
% 
% 
% 
% \subsubsection{\textbf{Results}}
% \begin{table*}[t]
% \caption{Performance of Models on different datasets}
% %\begin{center}
% %\scalebox{1.0}
% %{
% %\renewcommand*{\arraystretch}{3}
% \centering
% \begin{tabular}{p{.75cm}|rrr|rrr|rrr}
% %                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
% \multicolumn{1}{l}{}& \multicolumn{3}{c}{\textbf{Dataset $\mathcal{B_{BS}}$}}                                                                                                                            & \multicolumn{3}{c}{\textbf{Dataset $\mathcal{B_{NS}}$}}                                                                                                                                & \multicolumn{3}{c}{\textbf{Dataset $\mathcal{B_{DS}}$}}                                                                  \\ 
% \midrule
% {\textbf{Model}}    & {P}   & {R}   &{F1}     & {P}   & {R}   &{F1}    & {P}   & {R}   &{F1}   \\ 
% \midrule
% {\textbf{$\mathcal{M}$}} & {0.98} & {0.91} & {0.94} &\multirow{2}{*}{.98} & \multirow{2}{*}{.94} & \multirow{2}{*}{.96} & {.22} &{ .22} & {.22} \\ %\hline
% {\textbf{$\mathcal{M_{MS}}$}}    & { 1.0} & {0.94} & {0.98} & & & & {.82} &{.79}& {.8} \\ 
% \midrule
% \multicolumn{10}{c}{Performance increase(\%) of model $\mathcal{M_{MS}}$ over model $\mathcal{M}$}\\
% \midrule
% \multicolumn{1}{c}{}& { 2.04\%} & {2.76\%} & {2.65\%} & & & & {272.7\%} &{266.5\%}& {272.2\%}\\
% 
% \bottomrule
% \end{tabular}
% %}
% \label{table:performance_on_datasets}
% %\end{center}
% \end{table*}
% 
% In Table \ref{tab:comparison_M vs M_MS}, we showed performance of $\mathcal{M_{MS}}$ model on dataset $\mathcal{B_{MS}}$ using $10-cross~cross~validation$. Result shows, $\mathcal{M_{MS}}$ outperforms its predecessor $\mathcal{M}$ in all metrics. \textbf{Model improved Precision by 17.36\%, Recall by 12.82\% and F1-Score by 15.84\% from previous best model $\mathcal{M}$.} As we said earlier, this result is by no mean surprising rather expected. The only thing we could infer from this experiment is that this model learnt and fitted to the dataset better than model $\mathcal{M}$. \\  
% \textbf{In Table\ref{table:performance_on_datasets} We reported the performances of these model on newly created dataset $\mathcal{B_{BS}},~\mathcal{B_{NS}},~\mathcal{B_{DS}}$ . For, $\mathcal{B_{BS}}$ dataset, $\mathcal{M}$ model got .98 Precision and $\mathcal{M_{MS}}$ model got maximum 1 Precision}. This result indicates that $M_{MS}$ model performances did not drop from its predecessor $\mathcal{M}$. We could not take the subtle improvement into consideration without further investigation because we took only a small subset and both model got almost perfect value. Model $\mathcal{M_{MS}}$ also got higher Recall and hence F1-Score. As model has higher Precision and Recall at the same time, we can say- model is precisely predicting more positive instances than the other.\\
% We chose dataset $\mathcal{B_{NS}}$ because 96.71\% of data fell in this category. So performance on these dataset would provide us better insight about overall performances. \textbf{We found, models maintained high Precision of .98, Recall of .94 and F1-Score of .96. }
% This high value of performance metrics validates our previous experiment result, discussed in \ref{RQ3_approach}, and also proves the robustness of the models.\\
% We evaluated the models on dataset $\mathcal{B_{DS}}$ which provided us more conclusive evidence. Performances were shown in the Table \ref{table:performance_on_datasets}. Both models performed almost similarly until this point. \textbf{Model $\mathcal{M_{MS}}$ had a Precision of .82, Recall of .788 and F1-Score of .801 whereas model $\mathcal{M}$ had got only Precision of .22, Recall of .215 and F1-Score of .215 which are almost 73\% less.} As dataset $\mathcal{B_{BM}}$ only explored a few `cryptography' and `authentication' domains of security, model $\mathcal{M}$ only learnt these two domains and failed to identify others security related sentences. As a result, model $\mathcal{M}$ got low Precision, Recall and hence F1-Score. On the other hand, 510 new security sentences provided the model $\mathcal{M_{MS}}$ more insights about a few other security domains as well as those two domains which eventually led to higher Recall and Precision. This model misclassified many instances because of scarcity of various domain specific data in training dataset. Although, Model performed well on authentication and cryptography related sentences, but could not maintained that on other security domains.\\
% From the performances on three different dataset, we clearly state that model $\mathcal{M_{MS}}$ is performing better than other one and so it is our best performing model.\\
 
 
 

% \begin{table}[t]
%   \centering
%   \caption{BERT model performances on IoT dataset}
%     \begin{tabular}{lrrr} \toprule
%     \textbf{Model} & \textbf{P} & \textbf{R} & \textbf{F1} \\ 
%     \midrule
%     RoBERTa & 0.96 & 0.95 & 0.95\\
%     BERT extension & 0.95 & 0.94 & 0.95 \\
%     DistilBERT & 0.96 & 0.93 & 0.94 \\
%     Funnel BERT& 0.95 & 0.94 & 0.94 \\
%     Albert & 0.94 & 0.92 & 0.93\\
%     XLNet & 0.94 & 0.94 & 0.94 \\
%     Electra & 0.95 & 0.93 & 0.94 \\
%     SVM & 0.873 & 0.866 & 0.869\\
%     Logits & 0.87 & 0.861 & 0.865\\
    
    
%     \bottomrule
%     \end{tabular}%
%   \label{tab:performance-bert-iot}%
% \end{table}%


% \begin{table}[t]
%   \centering
%   \caption{BERT model performances on IoT+Opiner dataset}
%     \begin{tabular}{lrrr} \toprule
%     \textbf{Model} & \textbf{P} & \textbf{R} & \textbf{F1} \\ 
%     \midrule
%     RoBERTa & 0.92 & 0.94 & 0.93\\
%     BERT & 0.93 & 0.92 & 0.92 \\
%     DistilBERT & 0.93 & 0.92 & 0.92 \\
%     Funnel BERT & 0.92 & 0.93 & 0.92 \\
%     Albert & 0.92 & 0.88 & 0.9\\
%     XLNet & 0.92 & 0.92 & 0.92 \\
%     Electra & 0.9 & 0.92 & 0.91 \\
%     SVM & 0.874 & 0.872 & 0.873\\
%     Logits & 0.871 & 0.863 & 0.867\\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:performance-secbot-valsample}%
% \end{table}%



% \begin{table}[t]
%   \centering
%   \caption{BERT model performances on IoT+Opiner dataset}
%     \begin{tabular}{lrrr} \toprule
%     \textbf{Model} & \textbf{P} & \textbf{R} & \textbf{F1} \\ 
%     \midrule
%     DNN(IoT) & 0.904 & 0.854 & 0.876\\
%     CNN(IoT) & 0.907 & 0.866 & 0.885 \\
%     LSTM(IoT) & 0.913 & 0.885 & 0.898 \\
%     Bi-LSTM(IoT) & 0.914 & 0.867 & 0.889 \\
%     \midrule
%     DNN(IoT+Opiner) & 0.899 & 0.886 & 0.892\\
%     CNN(IoT+Opiner) & 0.884 & 0.915 & 0.899 \\
%     LSTM(IoT+Opiner) & 0.928 & 0.890 & 0.908 \\
%     Bi-LSTM(IoT+Opiner) & 0.907 & 0.885 & 0.895\\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:performance-secbot-valsample}%
% \end{table}%
 

\subsection{Misclassification Analysis of SecBot+ (RQ4)}\label{sec:misclassification-analysis-secbot+}
We do a qualitative study of the misclassifications of the best performing model (i.e., SecBot+) to detect security aspect in IoT discussions. 
The purpose is to learn about the possible avenues for future improvement of the model. 
\subsubsection{Approach} In our validation sample of 984 sentences, SecBot+ was wrong in 69 cases (false positive or false negative). We 
manually analyze all the 69 sentences to determine the reason for misclassification. The manual analysis process consisted of three 
stages. Both of the authors consulted together (over Skype) on all 69 sentences to give a textual label that could explain the 
reason of misclassification. For example, the following sentence is erroneously labeled as 1 (i.e., contains security discussion) by SecBot+ \emt{There could still be an input which unsets and sets your input pin faster your loop can detect it so it's not bulletproof.} 
After careful comparison of this sentence with other sentences in our validation sample, we determine that the misclssification is due to the ambiguity in context, which 
arose due to the presence of `bulletproof' and `input' in the sentence. We label the misclassification reason as `Ambiguous Context'.

The analysis of 69 sentences in the validation sample offers us valuable insights into 
the error categories of SecBot+, but the sample of 69 sentences could be too small to feel confident of the derived error categories. We thus analyzed another 132 sentences 
from our combined dataset of 5,297 sentences as follows. We applied a 10-fold cross validation on our entire 
combined dataset following steps similar to \sec\ref{sec:opiner-dataset-performance-approach}. 
As such, we were able to use the entire 5,297 sentences training and testing. At the end of the 10 iterations, we find a total of 132 misclassifications  in the entire 
5,297 sentences by the RoBERTa model used for SecBot+. We then manually analyze all the 132 sentences following approach similar to the validation sample above. We report the 
misclassification labels on the the total 132 + 69, i.e, 201 sentences.  

\subsubsection{Results} In \tbl\ref{tab:performance-10fold-combined}, we show the performance of all studied models including RoBERTa (i.e., the deep learning algorithm 
for SecBot+ in \sec\ref{sec:rq-secbotplus-dev}). Out of all the models, RoBERTa still performed the best in terms of F1-score and AUC score. The F1-score 
of RoBERTa is 0.912 and the AUC score is 0.961. The second best model is BERT with an F1-score of 0.910 and an AUC score of 0.946. Both 
RoBERTa and BERT show improved performance in the combined dataset than the validation sample. Overall, all the deep learning models still show 
better performance the baseline shallow learning models, which confirm the findings from the validation sample that the deep learning models 
are better suited to detect security aspects in IoT developer discussions. 
\begin{table}[t]
  \centering
  \caption{Performance of Studied Models on Combined Dataset after 10-fold Cross Validation}
    \begin{tabular}{llrrrrr}\toprule
    \multicolumn{1}{l}{\textbf{Model Type}} & \textbf{Model Name} & {\textbf{P}} & {\textbf{R}} & {\textbf{F1}} & {\textbf{Acc}} & {\textbf{AUC}} \\
    \midrule
    {Baseline} & SVM   & 0.812 & 0.89  & 0.848 & 0.96  & 0.93 \\
          & Logit & 0.801 & 0.891 & 0.843 & 0.958 & 0.93 \\
          \midrule
    {Seq2Seq} & LSTM  & 0.861 & 0.879 & 0.87  & 0.967 & 0.929 \\
          & Bi-LSTM & 0.861 & 0.849 & 0.854 & 0.966 & 0.914 \\
    \midrule
    {Transformer} & BERT  & 0.92  & 0.904 & 0.910  & 0.978 & 0.946 \\
          & \bf{Re-trained SecBot+ (i.e., RoBERTa)} & 0.888 & 0.939 & \bf{0.912} & 0.977 & 0.961 \\
          & XLNet & 0.871 & 0.929 & 0.898 & 0.974 & 0.954 \\
          & ALBERT & 0.91  & 0.885 & 0.897 & 0.974 & 0.936 \\
          & DistilBERT & 0.895 & 0.911 & 0.901 & 0.975 & 0.947 \\
          \bottomrule
    \end{tabular}%
  \label{tab:performance-10fold-combined}%
\end{table}%
\begin{figure}[t]
	\centering\begin{tikzpicture}[scale=0.3]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=150,
        color={black!0, black!10, black!20, black!30},
        ]
        {
            13.4/\bf{Implicit Context}\\(13.4\%S 27S),
            5.5/\bf{Code/Text Parsing Error}\\(5.5\%S 11S), 
            38.8/\bf{Ambiguous Context}\\(38.8\%S 78S),
            42.3/\bf{Ambiguous/Unknown Keywords}\\(42.3\%S 85S)
        }
    \end{tikzpicture}
	\caption{Distribution of SecBot+ error categories in the total 201 sentences (S) from validation sample and combined dataset}
	\vspace{-2mm}
	\label{fig:error-category-total}
\end{figure}
\begin{figure}[t]%[!htb]
  \centering
  \vspace{-10mm}
  \includegraphics[scale=.45]{images/ErrorLabelsMod.pdf}
  \vspace{-10mm}
  \caption{Distribution of the four error categories in the combined dataset and the validation sample}
  \label{fig:error-distribution}
\vspace{-3mm}
\end{figure}

In \fig\ref{fig:error-category-total}, we show the misclassification categories in to the total 201 sentences collected from the validation sample and the combined dataset. 
Overall, we find four error categories: \begin{inparaenum}
\item Ambiguous/Unknown Keywords, 
\item Ambiguous Context, 
\item Implicit Context, and 
\item Code/Text Parsing Error.
\end{inparaenum} The most observed error category is `Ambiguous/Unkown Keywords', which we observe in 42.3\% of all 201 sentence (i.e, 85 sentences). 
The category `Ambiguous Context' is observed the second most times (38.8\% sentences), followed by the category `Implicit Context' (13.4\% sentences), and 
Code/Text Parsing Error (5.5\% sentences), respectively. In \fig\ref{fig:error-distribution}, 
we break down the distribution of misclassification categories by the validation sample and the combined dataset. 
The distribution of the top three categories (i.e., Ambiguous/Unknown Keywords, Ambiguous Context, and Implicit Context) are almost similar in both the validation sample and 
combined dataset. Out of the total 11 sentences for which we observed `Code/Text Parsing Error', four of those are found in the combined dataset and seven are 
found in the validation sample. We discuss the error categories below.

\begin{inparaenum}[(1)]
\item \bf{Ambiguous/Unknown Keywords.} These errors occurred due to the presence of security-specific keywords that are not observed in the training data (i.e., unknown keywords) or  
Such errors also occurred when a keyword was predominantly found to be associated with security-specific sentences during training phases, 
but in the errorneous cases the keyword was found in a non-security 
specific scenario. Consider the sentence \emt{You could buy antenna which meets requirement of your gateway and LoRaWAN specification.} SecBot+ labeled this sentence as 1 (i.e., security), 
but the underlying scenario is about the setting up of an antenna in an IoT device. SecBot+ was confused due to the presence of keyword `gateway', which is predominantly found in the 
security-specific sentences during training. Similarly, SecBot+ erroneously labeled the following sentence as 1 due to the ambiguous presence of keyword like `lock', \emt{My issue seemed to be that the Pi was getting locked into a host-state while using the OTG micro-USB to USB adapter and thus couldn't receive any commands over the "ethernet" USB connection.}    

\item \bf{Ambiguous Context.} These errors occurred when the underlying context can be too ambiguous to properly detect the security aspect. Such ambiguity occurred because more 
information from surrounding sentences were needed. Consider the following sentence \emt{Voice Recognition means identification of the person talking and is frequently misapplied to mean "Speech Recognition" - identification of what is being said.}. 
SecBot+ labeled the sentence as 0, while it is 1 in the manual label. This is because the context is about the secure/private access to an IoT device 
via voice recognition. While the sentence attempts to differentiate between `Speech' and `Voice' recognition, the manual labeling phase still considered it as related to security discussions. 

\item \bf{Implicit Context.} SecBot+ was unable to discren underlying security context, when it was implicit. Consider the following sentence \emt{User agents and clients must adjust accordingly when a 301 redirect is given so that future requests for the same URL won't be requested in favor of the permanent redirect.} 
Here, user agents are redirected to prevent unauthorized requests to a specific URL. Such security-specific information is implicit in the sentence. As such, 
SecBot+ labels it as 0, whereas the benchmark manual label is 1. Similarly, the following sentence also denotes security-specific information implicitly for the Raspberry Pi device \emt{On-premises managed instances (which is what a Raspberry is after it's registered) are not supported by Session Manager today.} 

\item \bf{Code/Text Parsing Error.} These errors are very few compared to the other three categories. They occurred due to the inability of the tools used in the model to 
properly parse code or textual contents in the sentence. For example, SecBot+ erroneously labels the following sentence as 0, even though it is about the enablement 
of secure socket layer (SSL) in Raspbian Stretch device \emt{The version of Openssl on Raspbian Stretch is 1.0.2, but according to Openssl website, these versions should be binary compatible (https://www.openssl.org/policies/releasestrat.html).} 
While SecBot+ knew from training that SSL is related to security aspect, SSL in this sentence is denoted as Openssl, which is not known to SecBot+. Similarly, 
SecBot+ is unable to determine security threats related to input injection noted in the code block that is provided as texts in this sentence \emt{In Package tag add \ldots In Capabilities add \ldots <rescap:Capability Name="inputInjection" /><rescap:Capability Name="inputInjectionBrokered" />}. 
\end{inparaenum}  


==> detectIoTSecurityIST.tex <==
\section{Automatic Detection of IoT Security Aspect}\label{sec:results-aspect-detection}
We answer four research questions during our investigation on the effectiveness of deep learning models to detect security aspects in developer discussions:
\begin{enumerate}[leftmargin=30pt, label=\bf{RQ\arabic{*}.}]
%  \item How do the deep learning models perform to detect security aspects in Opiner API review dataset? (\sec\ref{sec:performance-api-review-dataset})
  %\item Can the advanced transfoer models offer improved performance to detect security aspects in Opiner benchmark? (\sec\ref{sec:rq-bert-opiner-data})
%  \item Can the models trained on API review dataset show similar performance in IoT discussions?  (\sec\ref{sec:rq-secbot-assess-iot})
  %\item Can the models be further improved by re-training on labeled data from IoT security discussions? (\sec\ref{sec:rq-secbotplus-dev})
  \item How do the deep learning models perform to detect IoT security aspects in the benchmark?
  \item What are the error categories in the misclassified cases of the best performing model? (\sec\ref{sec:misclassification-analysis-secbot+})
  \item Can a SE-specific word embedding help improve the performance?
  %\item Can the Performance of the BERT-Models Be Further Improved Using SE-Specific Embedding? 
\end{enumerate}
% The answer to first research question (RQ1) helps us to determine whether deep learning models can outperform the shallow learning models in Opiner for an already available 
% benchmark dataset of API review aspects. The API review dataset in Opiner does not have any sentences/posts picked from our 53K IoT posts. 
% While security discussions are prevalent across diverse computing paradigms, the nature of their discussions (e.g., the vocabularies, contexts) could 
% differ between and among the domains. The second research question (RQ2) then attempts to find out whether security aspect classification model trained on API review 
% dataset can perform well to detect security discussions in our IoT dataset. Intuitively, a good performance in such cross-data setting denote that security discussions 
% follow similar patterns between the two IoT and non-IoT (e.g., API review dataset) datasets in our study. The third research question (RQ3) aims to answer 
% whether and how by adding IoT-specific security discussions into the API review dataset would offer improved performance for the security aspect detection models. 
% The last research question (RQ4) offers a qualitative perspective on the misclassifications of the best performing classification model by analyzing the error categories. 
% Such analysis can help determine the causes of misclassifications and possible venues of further improvement in the security aspect detection in IoT developer discussions.    
\subsection{Performance Metrics} \label{sec:performance-metrics}
We analyze the performance of the classification models for security aspect detection using five standard metrics in 
information retrieval~\cite{Manning-IRIntroBook-Cambridge2009}: Precision (P), Recall (R), F1-score (F1), Accuracy (Acc) and Area Under the Curve (AUC).
\begin{itemize}[leftmargin=20pt]
  \item Precision (P) is the fraction of sentences labeled `HasSecurity' (i.e., the sentence contains security discussions) out of all the sentences labeled as `HasSecurity'. 
  \begin{equation}
  P  = \frac{TP}{TP+FP}
  \end{equation}
Here TP = Correctly classified a sentence as containing discussion about security, FP = Incorrectly classified as containing discussion about security,   
  \item Recall (R) is the fraction of all `HasSecurity' sentences that are successfully identified out of all sentences that contain security discussions.
  \begin{equation}
	R = \frac{TP}{TP+FN}
  \end{equation}
  Here FN = Incorrectly classified as not containing discussion about security.
  \item F1-score is the harmonic mean of precision (P) and Recall (R). 
  \begin{equation}
	F1 = 2*\frac{P*R}{P+R}
  \end{equation}
  \item Accuracy (A) is the fraction of all correctly classified out of all records.
  \begin{equation}
	Acc = \frac{TP + TN}{TP + TN + FP + FN}
  \end{equation}
  Here TN = Correctly classified as not containing discussion about security.
  \item AUC (Area Under the Curve) is the area under the Receiver Operating Characteristics (ROC) curve. An ROC curve is a graphical plot to illustrate the ability of a binary classifier (such as ours) 
  The ROC curve is plotted by taking ratio of TPR (True Positive Rate) against FPR (False Positive Rate) at various classification probability threshold (e.g., a probability of 1.0 will most likely denote a 
  100\% TPR and 0\% FPR, while a probability of 0.0 will most likely result the opposite). We calculate TPR and FPR and use those to calculate AUC as follows . 
  \begin{eqnarray}
  TPR = \frac{TP}{TP + FN}, ~
  FPR = \frac{FP}{FN + TP}, ~
  AUC = \int_{x = 0}^{1} {TPR}({FPR}^{-1}(x))dx
  \end{eqnarray}
  %\item MCC  
\end{itemize}
F1-score and AUC are preferred over metrics like accuracy (A) when evaluation dataset is imbalanced. For example, 
our API review dataset is imbalanced with lower number of sentences labeled as 1 (i.e., `HasSecurity' = 1) than sentences labeled as 0.  
Following standard practices in Literature~\cite{Zhang-SentimentDetectionSEBERT-ICSME2020,Uddin-OpinionValue-TSE2019}, 
we use F1-score to determine and report the best model. 



% 
% \begin{table}[t]
%   \centering
%   \caption{Summary stats for Opiner Dataset}
%     \begin{tabular}{rrrr}\toprule
%     \midrule
%     {\textbf{Total T}} & {\textbf{\#Security S}} & {\textbf{\%S/T}} & {\textbf{Non-Security}} \\
%     \midrule
%     4297  & 163   & 3.8\% & 4134 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:opiner-details}%
% \end{table}%


% 
% 
% In Machine Learning, dataset is divided into two or three subsets, training,
% validation, and testing. Model is trained on training dataset, tuned on
% validation dataset, and tested on testing dataset. Mainly, testing and
% validation dataset are used to limit model from getting overfitted and tuning
% the hyperparameters respectively. This strategy works fine when dataset is large
% but often struggles when dataset is small as training instances are deficient
% compared to model's parameters and thus, model underfits. Model needs
% substantial training data to overcome underfitting and at the same time,
% validation data to find the best parameter as well as best model, and also
% testing dataset to eschew underfitting. We need a middle ground, which seems a
% bit contradictory as well, where all requirements are met without compromising.
% Here comes $k-fold~cross~validation$\cite{inproceedings} to rescue. The idea is
% to divide the dataset, $D$, into $k$ disjoint folds, $D_i,~i=1...k$, of
% approximately equal size.
% $$D_i\cap D_j=\phi~~~\forall~i,j\in k~and ~i\ne j $$
% $$D_1\cup D_2\cup...\cup D_k = D$$
% To avoid overfitting, model is trained $k$ times, each time one of the $k$ folds are held out as validation set and rest of the $k$ folds are used as training set. The value of $k$ is a hyperparameter. This technique is quite effective in learning with small balanced dataset but could suffer from undersampling if dataset is imbalanced, like ours. Stratified random sampling, equally divides dataset into homogeneous subsets before sampling, can overcome the undersampling problem. Thus, we used \textbf{stratified} $k-fold~cross~validation$. We set \textbf{k as 10}, a value that has been found through experiment.\\
% 

\begin{table}[t]
\centering
\caption{Hyperparameters of the deep learning models after fine tuning}
\begin{tabular}{p{2cm}l|rrrrr}
\toprule
\bf{Type} & \textbf{Model}& \bf{Batch Size} & \bf{Epochs}  & \bf{Optimizer} & \bf{Loss Functions} & \bf{Learning Rate}\\ 
\midrule
\multirow{2}[0]{*}{seq2seq} &  LSTM & 64 & 50 & Adam & binary-crossentropy & 2e-3\\ 
& Bi-LSTM & 64 & 20 & Adam & binary-crossentropy & 2e-3\\
 \midrule
\multirow{5}[0]{*}{Transformer} & BERT & 32 & 3 & Adam & binary-crossentropy & 3e-5 \\
& RoBERTa & 32 & 3 & Adam & binary-crossentropy & 1e-5 \\
& XLNet & 32 & 3 & Adam & binary-crossentropy & 3e-5 \\
& ALBERT & 32 & 3 & Adam & binary-crossentropy & 1e-5 \\
& DistilBERT & 16 & 3 & Adam & binary-crossentropy & 3e-5\\
 %FunnelBERT & funnel-transformer/small-base &12& 768 & 12 & 115M \\
 %ELECTRA& google/electra-small-discriminator&  12&	256&12 &	14M\\
\bottomrule
\end{tabular}
%}
\label{dllParamAPIReview} 
%\end{center}
\end{table}


\subsection{Performance of Deep Learning Models on IoT Benchmark (RQ1)}
\subsubsection{Approach} approach
\subsubsection{Results} results

\subsection{Error Categories of the Best Performing Deep Learning Model on IoT Benchmark (RQ2)}
\subsubsection{Approach} approach
\subsubsection{Results} results

\subsection{Impact of SO Specific Embedding on Performance (RQ3)}
\subsubsection{Approach} approach
\subsubsection{Results} results


==> empiricalStudy.tex <==
\section{Empirical Study of Security Aspects in IoT Developer Discussions} \label{sec:results}
The superior performance of our developed SecBot+ model allows us to reliably use this model to
automatically collect IoT-related security sentences from SO. Such mined data
then can be used to conduct empirical studies like understanding the types of
security topics IoT developers are discussing in SO. In this section, we prepare a dataset of all IoT
security sentences from our 53K IoT posts and use the dataset to answer the following research questions: 
\begin{enumerate}[start=4, leftmargin=30pt, label=\bf{RQ\arabic{*}.}]
  \item What are topics in the IoT security discussions collected from SO? (\sec\ref{sec:rq-iot-sec-topic})
  \item How do the IoT security topics evolve? (\sec\ref{sec:rq-iot-sec-topic-evolve})
\end{enumerate} 
The first research question (RQ5) aims to understand the types of topics found in the sentences labeled as security by SecBot+. 
Such information can inform of the prevalence of specific security topics in IoT developer discussions, which we normally have to find by conducting 
surveys of IoT developers. The second research question (RQ6) investigates the evolution of the IoT security topics found in RQ5. Such information 
can help to understand whether and how the popularity of specific IoT security topics may be changing over time. Such evolution information can be hard 
to find from any other sources and so could be valuable to understand IoT developer interests and problems over time. 
%\subsection{IoT Security Data Collection}\label{sec:iot-security-data}

% \nd\bf{Topic Modeling.} We used Latent Dirichlet Allocation(LDA) algorithm\cite{blei2003latent} available under the MALLET library in \href{https://radimrehurek.com/gensim/models/ldamodel.html}{Gensim}. LDA takes a set of texts as a input and outputs a list of topics to group the texts into K topics. This K is a hyperparameter of the algorithm. To get optimal value of K, we used standard practice as originally proposed by Arun at el\cite{Arun-OptimalTopic-AKDD2010}. This approach suggests that optimal number of topics has the highest coherence among them, i.e., the more coherent the topics, the better topics can encapsulate the underlying concepts. To determine this coherence metric, we used standard c\_v metric available in Gensim package. To determine our optimal number of topic, we used grid search technique. We fist selected a set of values for hyperparamter, K. Then we run our MALLET LDA algorithm for each value of K and measured the coherence metric. Finally, we chose the value of K that is associated with highest coherence score. In our experiment, we set K = {1,6,11,16,21,26,31,36,41,46} and got maximum coherence of .412 for K=11. Thus, we picked 11 as our optimal number of topics for dataset IoT Security discussion dataset.           

%\nd\bf{Topic Labeling.} 
% Then, we implemented
% bi-grams and tri-grams to get more meaningful words and applied lemmatization to
% get root words. Then we filtered unwanted parts of speech tag and again removed
% stopwords.

\subsection{IoT Security Topics in Developer Discussions (RQ4)}\label{sec:rq-iot-sec-topic}
We automatically detect security topics in the sentences labeled as security-specific by SecBot+ in our IoT dataset.  
\subsubsection{Approach} \it{\ul{First}}, we apply SecBot+ on the entire 672,678 sentences that we collected from our 53K
IoT posts (\sec\ref{sec:iot-data-collection}). SecBot+ returned 34,270 sentences
as 1, i.e., those contain security discussions. \it{\ul{Second}}, We preprocess this dataset as
follows. We removed stopwords, short tokens and letter accents. The stopwords are collected from 
NLTK~\cite{website:nltk}. We applied lemmatization on sentences to get root form 
of each word. \it{\ul{Third}}, we fed the preprocessed sentences into the topic modeling algorithm Latent Dirichlet Allocation (LDA)~\cite{blei2003latent} 
available via Gensim~\cite{Radim-gensim-LREC2010}. LDA takes a
set of texts as a input and outputs a list of topics to group the texts into K
topics. This K is a hyperparameter of the algorithm. To get optimal value of K,
we used standard practice as originally proposed by Arun at
el\cite{Arun-OptimalTopic-AKDD2010}. This approach suggests that optimal number
of topics has the highest coherence among them, i.e., the more coherent the
topics, the better topics can encapsulate the underlying concepts. To determine
this coherence metric, we use the standard c\_v metric as originally 
proposed by R\"{o}der et al.~\cite{Roder-TopicCoherence-WSDM2015}. We use the topic coherence metric as available in 
Gensim package~\cite{Radim-gensim-LREC2010}. To determine our optimal number of topic, we used grid search technique. We fist
selected a set of values for K. Then we run our LDA
algorithm for each value of K and measured the coherence metric. Finally, we
chose the value of K that is associated with highest coherence score. In our
experiment, we set K = {1,4,8,9, 10,11, 12, 16,20,24,28,32, 36, 40} and got maximum coherence
score for K = 12. Thus, we picked 12 as our optimal number of topics. LDA also uses two hyper parameters $\alpha$ and $\beta$ to control the 
distribution of words in topics and the distribution of topics in posts. Biggers et al.~\cite{Briggers-ConfigureLDA-EMSE2014} 
conducted an empirical study on the configuration of LDA for software feature analysis and found that 
\emph{``$\alpha$ and $\beta$ value [change] have little influence on the accuracy of the LDA [topic modeling]''}.
Following previous work~\cite{Barua-StackoverflowTopics-ESE2012,Bagherzadeh2019,Ahmed-ConcurrencyTopic-ESEM2018,Briggers-ConfigureLDA-EMSE2014,Rosen-MobileDiscussionSO-EMSE2016,YangLo-SecurityDiscussionsSO-JCST2016}, we thus use standard 
values $50/K$ and 0.01 for the two hyper parameters. \it{\ul{Fourth}}, we label each topic a name by manually
analyzing a random sample of at least 50 sentences per topic. We did not limit
ourselves to a finite number of sentences per topic during the labeling to
ensure that the assigned label is reliable. The first and second authors labeled
the topics by consulting together. For example, the following sentence is about the configuration of firewall and target remote device for 
authentication, \emt{\ldots you can check the configuration of target device and firewall setting.And more,I want to add that,please note the configuration of Authentication Mode.You should set it as "Universal(Unencrypted Protocol)".Use the mode whenever you are deploying to a remote device.} 
Another sentence assigned to the same topic is \emt{Looks like a list of random words, maybe passwords for a brute-force attack:  \ldots curious2s \ldots curious2saab95}. 
We thus label the topic as `User/Device Authorization'. Similarly the following the topic labeled as `Secure Transaction' has sentence related to secure communication/transaction, e.g., 
\emt{\ldots Scan barcodes using Goggles to get product information} or \emt{When the card is scanned, the data from the database will be retrieved and show to the interface screen, I have 2 RFID which is located in separated doors \ldots}. 
\it{\ul{Fifth}}, we assign each topic a category, where a
category denotes a higher order grouping of the topics. For example, we assign the topics `User/Device Authorization' and `Crypto/Encryption Support' to category `Software', because 
the topics contain discussion about the support of software in IoT devices to ensure security. The topic `Secure Transaction' is assigned to the category `Network, because 
it contains discussions about the securing of transactions/communication between IoT devices/services over network. 


\begin{figure}[t]
	\centering\begin{tikzpicture}[scale=0.35]-
    \pie[
        /tikz/every pin/.style={align=center},
        text=pin, number in legend,
        explode=0.0, rotate=120,
        color={black!0, black!10, black!20},
        ]
        {
            35.0/\bf{Network}\\(35.0\%S 4T), 
            57.6/\bf{Software}\\(57.6\%S 7T),
            7.4/\bf{Hardware}\\(7.4\%S 1T)
        }
    \end{tikzpicture}
	\caption{Distribution of sentences (S) and topics (T) per topic category}
	\vspace{-2mm}
	\label{fig:topic-cat-dist}
\end{figure}
% 
%  \begin{figure}[t]
% 	\centering\begin{tikzpicture}[scale=0.4]-
%     \pie[
%         /tikz/every pin/.style={align=center},
%         text=pin, number in legend,
%         explode=0.0,
%         color={black!40, black!20, black!0},
%         ]
%         {
%             62.29/\bf{Software Topic Category}\\(62.3\%Q 7T),
%             28.52/\bf{Network Topic Category}\\(28.5\%Q 3T),
%             8.79/\bf{Hardware Topic Category}\\(8.8\%Q 1T)
%         }
%     \end{tikzpicture}
% 	\caption{Distribution of sentences and topics per topic category}
% 	\vspace{-5mm}
% 	\label{fig:topic-cat-dist}
% \end{figure}


\begin{figure}[t]%[!htb]
  \centering
  \includegraphics[scale=.5]{images/TopicDistribution.pdf}

  \caption{Distribution of IoT Security Topics by Total \#Sentences (S = Software Topic Category, N = Network, H = Hardware)}

  \label{fig:ditribution_iot}
\vspace{-5mm}
\end{figure}

\subsubsection{Results} We found 12 IoT security related topics which are grouped into
into three high-level categories: Software, Network, and Hardware. \fig\ref{fig:topic-cat-dist} shows the distribution of
these three high-level categories. The Software category 
contains the most number of topics (7) and covers more than 57\% of all sentences. In \fig\ref{fig:ditribution_iot}, 
we sort the 12 topics based on the distribution of sentences in a descending order. 
The topic `User/Device Authorization' from the Software category 
covers the highest number of sentences (13.4\%). This topic contains 
discussions about developers' problems to setup up permission for an IoT device using various 
security measures like certificate installation, role-based access control, etc. (e.g., \dq{36904875}). $Q_i$ denotes a question with an ID $i$ in SO. The 
topic `Framework/SDK-based Security' from the Software category 
covers the lowest number of sentences among all topics (5.9\%). It contains
discussions about the vulnerability of specific approach in frameworks (e.g.,
safe-list approach in .NET framework \dq{3625178}). The other five topics in Software Category
are: \begin{inparaenum} \item Documentation and usages of Cryptography/Encryption support (9.4\%), 
\item Storage and Database management system (7.8\%), \item Implementation of secure
digital signature (7.4\%), \item  Mitigation techniques of
vulnerabilities/attacks in IoT devices (6.9\%), and \item Secure data management (6.7\%).
\end{inparaenum}

The Network category has the second most number of topics (4) and it covers 35\% of all sentences. 
Three of out the four topics under the Network category are also among the top four topics (each with around 9\% of sentences). The first two topics are `Secure Connection Configuration' and `Secure Transaction' that contain discussions about ensuring security over secure payments and secure copy/transfer of digital files via/among IoT devices. The other two network topics are 'IoT Hub Federation' and 'Secure Communication'. Questions in both topics concern about cloud-based setup of IoT devices, e.g., using Azure/AWS/Google cloud. IoT hub is a managed service in the cloud that acts as a central messaging service to allow bi-directional communication between an IoT application and 
the smart devices it manages (e.g., connect to MQTT with authenticated Cognito credential \dq{51093154}).

The Hardware category has one topic on the secure configuration and usage of
Microchip/Bluetooth (7.4\%). This topic contains discussions of programming and
configuration challenges IoT developers face while using Bluetooth/BLE/Microchip
interfaces in their IoT devices to setup a service (e.g., setup a barcode
scanner in rpi2 to verify coupon \dq{30721018}).
 
% 
% 
% 
%   has highest
% coverage of sentences (around 52.9\% of sentences and 6 topics), followed by
% Network (around 38.3\% of sentences and 4 topics), Hardware(around 8.8\% and
% only 1 topic). We also reported 11 topics wise distribution of sentences in
% Figure \ref{fig:ditribution_iot}. `User/Device Permission' related topic
% discussed in highest numbers of sentences (4675 sentences, around 15.5\% of
% total sentences), followed by `IoT Hub Federation' (3066 sentences, around
% 10.2\% of total sentences), `Iaas Setup/Conf' (3010 sentences, around 10\% of
% total sentences), `Secure Transactions' (2965 sentences, around 9.8\% of total
% sentences), `Bluetooth/Microchip Connection \& Communication' (2653 sentences,
% around 8.8\% of total sentences), `Framework/SDK Security' (2618 sentences,
% around 8.7\% of total sentences), `Secure Copy/Transfer' (2536 sentences,
% around 8.5\% of total sentences), `Vulnerabilities/Attacks' (2361 sentences,
% around 7.8\% of total sentences), `Secure Digital Signature' (2229 sentences,
% around 7.4\% of total sentences), `Authentication/Database Management' (2143
% sentences, around 7.1\% of total sentences), `Crypto/Encryption Support' (1963
% sentences, around 6.5\% of total sentences). Now, we analysis the topics by
% three categories below. We included 4 topics under this Network category: IoT
% Hub Federation, IaaS Setup/Configuration, Secure Copy/Transfer, Secure
% Transactions. In Hardware
% category, we put only Bluetooth/Microchip Connection and Communication. In our
% largest category- Software, contained 6 topics- User/Device Permission, Framework/SDK Security, Vulnerabilities/Attacks, Secure Digital
% Management, Authentication/Database Management, Crypto/Encryption Support.



\subsection{IoT Security Topics Evolution (RQ5)}\label{sec:rq-iot-sec-topic-evolve}
We investigate how the popularity of the three IoT security topic categories has changed over time by determining the total number of new sentences created per topic category 
over time. A new sentence can only be created if a new post is created. Therefore, the evolution of the topics over time offers us information of the relative popularity 
of the category and whether a category is discussed more over time than the other category.   
\subsubsection{Approach} For each of 34K security-related sentences in our dataset, we identify the ID of SO post from where 
the sentence is detected. We consider the creation time of the SO post to the sentence creation time. We group the 34K sentences by the three 
topic categories. For each category, we compute the total number of sentences created per six months based on the creation time. Following Wan et al.~\cite{Wan-BlockChainTopicSO-IEEETSE2019}, 
we report the 
evolution of IoT security topics using the metric Topic absolute impact. 
% two metrics: \begin{inparanum}[1]
% \item Topic absolute impact, and 
% \item Topic relative impact
% \end{inparanum}
Topic absolute impact is calculated as by determining the total number of sentences created per the 12 IoT topics every six months since 2008. 
We do this by first assigning each sentence to its most dominant topic, i.e., the topic with which the sentence show the highest correlation score. 
We then assign the creation time to a sentence as the creation time of the post where the sentence is found. Finally, for each topic, we put the sentences into 
time-buckets, where each bucket contains all sentences created within a time window (e.g., Jan 2009 till June 2009, etc.). 

%Topic relative imppact is calculated by taking   
% Following 
% Wan et al.~\cite{Wan-BlockChainTopicSO-IEEETSE2019}, we compute the absolute growth of each topic category as the number of new sentences 
% created per topic category per six months.  
% 
% \nd\bf{Step 1. Compute Topic Absolute Impact.} We apply topic popularity metrics as proposed in a previous work \cite{han2020programmers} to compute the popularity of a topic $z_k$ within corpus $c_j$ for a post $d_i$, where $i$ can be any topic within corpus $c_j$. Formally, the popularity of each topic is defined as:
% 
% \begin{equation}
% popularity (z_k,c_j) = \frac{|{d_i}|}{|c_j|}:dominant (d_i)=z_k, 1\le i \le c_j, 1\le j\le K
% \label{topicpoularity}
% \end{equation}
% 
% We apply LDA for corpus $c_j$ to get a set of K topics ($z_1$,.........,$z_k$). We denote the probability for a specific topic $z_k$ in a post $d_i$  as $\theta$($d_i$,$z_k$) to define the absolute impact metric of a topic $z_k$ in a month $m$ as: 
% 
% \begin{equation}
% impact_{absolute}(z_k;m) = \sum_{d_i=1}^{D(m)} \theta (d_i; z_k)   
% \label{absoluteeq}
% \end{equation}
% 
% \noindent where $D(m)$ is the  total number of posts in month $m$. We further refine this absolute-impact metric for a category $C$ for a specific month as:
% 
% \begin{equation}
% impact_{absolute}(C;m) = \sum_{z_k}^{C}impact_{absolute}(z_k; m)
% \label{absoluteeqsw}
% \end{equation}
% 
% The category $C$ belongs to four major category of IoT topic i.e., \textit{Hardware, Software, Network and Tutorial}. 
% 
% 
% 
% \nd\bf{Step 2. Compute Topic Relative Impact.} We use the relative impact metric to calculate the relative impact of IoT topic in a specific time, inspired from a previous work~\cite{han2020programmers}. We define the relative impact metric of a topic $z_k$ in $m$ as:
% 
% \begin{equation}
% impact_{relative}(z_k,m) = \frac{1}{|D(m)|}\sum_{d_i=1}^\theta(d_i; z_k) , 1\le i\le c_i 
% \label{relativeeq}
% \end{equation}
% 
% \noindent where $D(m)$ is the total number of posts in month $m$ that contain topic $z_k$. The $\theta$ shows the probability of particular topic $z_k$ for a post $d_i$. The relative impact metric estimates the proportion of posts for a specific topic $z_k$ relative to all posts in a particular month $m$. We also apply the relative impact metric on categories:
% 
% \begin{equation}
% impact_{relative}(C;m) = \sum_{z_k}^{C}impact_{relative}(z_k;m)
% \label{relativeeqsw}
% \end{equation}
% 
% \noindent where \emph{C} is the set of posts related to one of the  four major categories of IoT posts.

% To show how security related discussions evolved over
% the time, we created two charts: i) Relative Growth of Security Discussion in SO
% ii) Absolute Growth of Security Topics in Security Discussion. Relative growth of security measures the relative change in the total number of
% security related sentences compared to the change in the total number of
% sentences for the entire SO dataset.
%\subsubsection{Results} show and discuss how the topics are evolving over time, e.g., no of sentences per month per topic.\\
\begin{figure}[t]%[!htb]
 \hspace{-0.8cm}
  \includegraphics[scale=.7]{images/Popularity_count.pdf}
	\vspace{-5mm}
  \caption{\#New sentences per IoT security topic category each month}

  \label{fig:popularity_overtime}
\vspace{-5mm}
\end{figure}

% \begin{figure}[t]%[!htb]
%  
%   \includegraphics[scale=.55]{images/relativeGrowth.pdf}
% 	\vspace{-5mm}
%   \caption{\#New sentences per IoT security topic category each month}
% 
%   \label{fig:popularity_overtime}
% \vspace{-5mm}
% \end{figure}


\subsubsection{Results} Figure \ref{fig:popularity_overtime} show the absolute growth of the three IoT security 
topic categories over time by showing the number of new sentences per category each six months. While Software category 
has the most new sentences among the three categories, the Network category started to catch up starting from 2017. 
The number of discussions under Software shows an upswing in Dec 2012, when DeviceHub, a free open source machine
to machine communication (M2M) framework, was launched. Many discussions in Dec 2012 in our dataset are related to DeviceHub. 
Similarly, the realease of Riot.js, simple
component based UI, gave a spike in Software related
security discussions in 2014. Overall, the periods between June 2011 and June 2014 showcase the 
the rapid adoption of IoT-based SDKs/framekwors (e.g., rpi2 versions). 
IoT security concerns raised at the same time due to the 
emergence of ransomware like CryptoLokcer and banking Trojans. 

%  
% At the same time,  
% in 2013, due to emergence of CryptoLocker and attacks caused by banking Trojans
% discussion about software security had risen again specially in field of 
% encryption, digital security, and software vulnerabilities which drew attention
% of more security related discussions in subsequent years.
% We found most of the
% spike during period, 2012 to 2013, were related to this DeviceHub release.
%  Software discussions had shown a huge jump between January 2010 to
% January 2011 before a downward slops in between June,2011 and December,2011.
% Apart from this we found more upward slopes in between December 2011 to June
% 2013, December 2013 to June 2014, December 2015 to June 2016, December 2016 to
% June 2018 and December 2018 to June 2019. We further investigated to figure out
% reason behind this upward slopes. 

At the beginning of 2010, Network topic category got high priority due to internet
connectivity and cloud storage. A high spike is found at that time. Firebase, a real-time cloud database suited for IoT applications was released in May 2012. 
As such, we found many related security discussions across Network category during this time. Similarly, we found the release of IoT hubs like AWS IoT in 2015  
and IBM Watson IoT in 2017 contributed to many Network related discussions during the respective periods. Recently,
the emergence of online transaction and IoT cloud storage solutions also contributed to the increased popularity of Network category (\#new sentences). 

Hardware related discussions showed continuous growth over the years. Many
hardware supported security module like fingerprint lock, smart door, biometric
device, etc have emerged during our study period. We found the release of popular open source IoT hardware has
increased the rate of discussion about that hardware. For example, the release of
Intel Galelio back in mid 2012 produced a spike between June 2013 and December
2013. Similarly after the release of `Rasberry Pi 2' in February 2016 and
`Arduino Uno Wifi rev 2' in February 2017, spikes in curve were visible. 

% \begin{figure}[t]%[!htb]
%   \centering
%   \includegraphics[scale=.5]{images/relative_popularity.pdf}
% 
%   \caption{Relative Topic Popularity Evolution}
% 
%   \label{fig:relative_popularity}
% 
% \end{figure}
% 
% 
% 
% In Figure \ref{fig:relative_popularity} we showed relative changes of popularity
% of security discussion in three topics. We can see software security were most
% discussed in between October 2008 to December 2018 before Network related topics
% grabs the position. Software has a downward slops from January 2012 and
% continues to fall. Whereas both Network and Hardware showed upward slopes at
% that same period. After internet got accessible by common user and cloud storage
% had a huge private data at beginning of 2010, Network related security topics
% were discussed more frequently. Malicious attacks, cyber security,
% authentication, and etc sought attention of user and these related post were
% discussed during this period. Smart home, security lock and hardware-software
% collaborative apps and software got popularity in 2014. Hence security related
% Hardware discussions were posted and asked more frequently after 2014.

In summary, the evolution of IoT security topic categories and the subsequent topics can offer information into the new/emerging/existing 
IoT security tools and techniques real-world usage insights of their by the IoT developers. 
% In term
% of popularity this topics are never discussed as much as Network or Software but
% these discussions are increasing without any downfall from 2008 to 2019.




==> studied-models.tex <==
\section{Studied Deep Learning Models}\label{sec:studied-models}
The detection of security aspects in developer discussions was previously studied by Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019}, who investigated with 
two shallow learning models (SVM and Logistic Regression). We are aware of now studies that focused on the development of 
deep learning models to detect security aspect in developer discussions. In this section, we introduce a suite of deep learning models that we investigated to improve 
security aspect detection in developer discussions. The models can be broadly divided into two types:
\begin{enumerate}
  \item Deep learning Models which are found to offer superior performance for text classifications (e.g., language translation) 
  \item Transformer Models like the advanced pre-trained language models which are found to outperform other deep learning models for many text classifications (e.g., sentiment detection).
\end{enumerate}
\tbl\ref{tab:studied-models} presents the studied models. We discuss 
the architecture and features used in the studied models below. %studied seq2seq models in \sec\ref{sec:background-seq2seq} and the transformer models in \sec\ref{sec:background-transformer}.  

% Table generated by Excel2LaTeX from sheet 'models'
\begin{table}[t]
  \centering
  \caption{Studied Deep Learning Models}
    \begin{tabular}{p{2cm}lp{11cm}}\toprule
    {\textbf{Type}} & \textbf{Name} & \multicolumn{1}{l}{\textbf{Rationale to Study}} \\
    \midrule
    {RNN Models} & LSTM  & {Long Short Term Memory (LSTM) preserves history in sequences like word positions and occurrences, which is useful for text classification where context is important} \\
          & Bi-LSTM & {Bidirectional LSTM analyzes an input two ways - from past to future and from future to past. 
          This offers more contexts than LSTM (which is from past to future)} \\
    \midrule
    {Transformer Models} & BERT  &  BERT is designed to learn pre-trained contextual word representation by running of large volume of unlabeled texts. 
    The transformer mechanism allows the encoder and decoder to see the entire input sequence at once.
    \\
         & XLNet &  XLNet offers better training methodology and uses more data for pre-training than BERT, which could increase its accuracy in learning.
          \\
          & RoBERTa & RoBERT uses more data and computation power to learn from the data. It also offers better training methodology than BERT and XLNet. As a result RoBERTa outperforms both BERT and XLNet on benchmark datasets (e.g., GLUE)
           \\
          & Albert &  Albert architecture offers a light-weight version of BERT architecture, without suffering much on the text classification performance. 
          \\
          & DistilBERT & DistilBERT is also a lightweight version of BERT in terms of the learned architecture and word embedding, while retaining more than 95\% of BERT performance.
           \\
          %& FunnelBERT &  \\
          %& ELECTRA &  \\
          \bottomrule
    \end{tabular}%
  \label{tab:studied-models}%
\end{table}%

%We compare the performance of four traditional DL models against the state-of-the-art shallow learning models (Logit and SVM) 
%in Opiner to detect security aspect~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017}. 

\subsection{RNN Models}\label{sec:background-seq2seq}
\nd\bf{\ul{Studied Models.}} The seq2seq models for text classification learns words and their sequences from training data to determine how such a combination of 
words and their surrounding contexts could be useful to predict the labels given to the input data. Such models are found to be effective 
for text classification, because we often need more than one word to understand the underlying contexts. 
In this study, we investigated two of the most recent seq2seq models: \begin{inparaenum}[(1)]
\item Long Short Term Memory (LSTM)~\cite{Hochreiter-LSTM-NeuralComputation}, and 
\item Bidirectional LSTM (Bi-LSTM)~\cite{Huang-biLSTM-Arxiv2015}. 
\end{inparaenum} 

%Edited
% We investigate the performance of these models for sentiment classification task
% to get insight into model's validity for our case. Dang at el.\cite{Dang_2020}
% and Ain at el.\cite{Ain2017} showed comparative analysis of different deep
% learning models e.g DNN, RNN, and CNN for sentiment analysis across different
% datasets. Alharbi at el.\cite{ALHARBI201950} applied CNN, and LSTM and Abid at
% el.\cite{ABID2019292} applied Bi-LSTM, and CNN model for twitter sentiment
% classification. Hameed et al.\cite{bilstm_hameed} reported that Single-Layered
% BiLSTM Model performed better than other deep models for sentiment detection in
% short sentences. A short description of these model are given below-\\

%Edited

% DNN is a composition of input layer, output layer and hidden layers (and their
% neurons). Output of each layer is filtered by an activation function. Activation
% functions add non-linearity to the model which help it to learn complex
% relationship like the description of security-related problems in multiple
% connected words.
% CNN extracts multiple features including low level features which later feed on
% a pooling layer and finally a few dense layers do the classification task. Low
% level feature extraction makes CNN model effective in classification problems.
% For text classification CNN model is useful to extract hidden feature and
% context of the sentences.
% In text classification, semantics of words can be inferred based on insights
% about word co-locations \cite{semantics_text_classification}.
% CNN can get local semantic meaning of a sentence as it uses filter to go through
% the whole sentences but DNN ignores it. Recurrent neural network
% (RNN)~\cite{rnn-model} takes the words sequentially for a given input sentence.
% However, RNN has vanishing gradient problem~\cite{rnn-vanishing-gradient}. 
\begin{figure}
    \centering
    \includegraphics[scale=.3]{images/LSTM(Archi_Total).pdf}
    \caption{Used LSTM Architecture}
    \label{fig:LSTM Archi}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[scale=.35]{images/LSTM.pdf}
    \caption{A Single Long Term Short Memory(LSTM) Architecture}
    \label{fig:LSTM}
\end{figure}
\nd\bf{\ul{Model Architecture.}} Figure \ref{fig:LSTM Archi} shows the LSTM model in our experiment, which 
we adopted following standard LSTM architecture in the literature (e.g., Alharbi et al.~\cite{Alharbi-LSTM-CognitiveJournal2019}). This
architecture is consisted of a LSTM layer, two Dense layers, and a Flatten layer. At
first, it takes embedded sentences as input  and feeds into a LSTM of unit
size 64. LSTM is the core layer of this model that learns the context of
sentences. Then, a Dense layer of unit size 16 encodes the sentences into a
reduced dimension. A ReLU activation at the top of this Dense layer adds
non-linearity to the model that helps the model to learn complex pattern. Then,
a Flatten layer collapses the spatial dimensions of the sentences. Another Dense
layer of size 32 propagates the information of flattened output. Finally, a
Dense layer of unit size 1 makes prediction. Sigmoid activation ensures the
prediction are bound between 0 and 1. LSTM layer is the heart of this architecture, has a memory cell in its core
components. This memory cell stores the information of previous state of
training and this information leverages the model to learn context of the
sentences. Model makes prediction based on this stored information and the
information of current state. These states information get updated via gates to
enhance prediction performance. Gates are different from neural network that can
learn relevant information and update the state accordingly. This feature gives
extra edge over other deep models specially in sentence classification task.

Figure \ref{fig:LSTM} shows the system design inside a LSTM layer with  two cell states, three gates and a few activation functions. 
First, \textbf{forget gate$(f_t)$} decides the information of the
previous cell state$(c_{t-1})$ to be kept or discarded. It processes the
information of the previous hidden state $(h_{t-1})$ and current input$(X_t)$
through a sigmoid$(\sigma)$ activation function. These outputs are then
pointwise multiplied with previous cell state. This pointwise multiplication
means the amplification or diminishing of previous cell state. For example, if
the values of forget gate is close to 1, the values of previous cell state are
mostly retained in the output of multiplication step e.g. ``remember the past''.
On contrary, if the values of forget gate is close to 0, the previous cell state
values are scaled down e.g. ``forget the past''. So, forget gate is learned so
that it's outputs are close to 0 when current input is relevant to the objective
and close to 1 when current input is irrelevant. Next, \textbf{input gate$(i_t)$} decides the information of new memory
state(\~{c}$_t$) to be added into current cell state($c_t$). New memory network
extract feature to encode more meaningful data to the LSTM. Like forget gate,
both the input gate and new memory network take previous hidden state and
current input as inputs. New memory network is tanh activated that generate new
memory state and input gate is sigmoid activated like forget gate. This new
memory state represents the context of current input based on previous hidden
state. Then, output of input gate is multiplied with new memory state to
determine the magnitude of the new information that is added to current cell
state. Finally, \textbf{output gate($o_t$)} decides the information of the cell state
is used to update hidden state$(h_t)$ and produce final output($Y_t$). Like
input gate, output gate is sigmoid activated that takes previous hidden state
and current input as inputs. Then, this gate is multiplied with tanh activated
current cell state to produce final output and hidden state. Tanh activation
pushes the current cell state to be between -1 to 1 that helps the model to
learn faster. 

\begin{figure}
    \centering
    \includegraphics[scale=.25]{images/BiLSTM(Archi).pdf}
    \caption{Used Bi-LSTM Architecture}
    \label{fig:BiLSTM Archi}
    \vspace{-2mm}
\end{figure}
Figure \ref{fig:BiLSTM Archi} shows the architecture we used for Bidirectional LSTM, following 
standard literature (e.g. Hameed et al.~\cite{Hameed-BiLSTM-IEEEAccess2020}). This
architecture is almost identical except the core LSTM layer. Instead of a single LSTM
layer, this model has two different LSTM layers of unit size 64 that are fed
same input. A LSTM takes the input in forward manner and other one takes the
input in backward manner. This means that model can learn the context from both
direction. In forward LSTM, model learn the context of forward direction and
similarly, in backward LSTM, model learn the context of backward direction.
Later these two contexts are concatenated to get overall context of the
sentences. A Dense layer of unit size 64 squeezed the context into lower
dimension and a Flatten layer collapses the spatial dimension. Finally, two
Dense layer of unit size 32 and 1 respectively make the prediction.

\nd\bf{\ul{Model Features.}} Bag of Words (BoW) and word embedding are the most
commonly used for feature selection. We used GloVe embedding as feature
selection technique for LSTM and Bi-LSTM. The BoW technique suffers from sparsity problems. Word
embedding, another text encoding technique, represents a
text or a document based on the context more precisely. Word embedding has a upper
hand compared to bag of words but it takes much longer to train. 
Several open source pretrained embedded models are available. \href{https://nlp.stanford.edu/projects/glove/}{GloVe}\cite{pennington-etal-2014-glove} is an open
source pretrained word embedded matrix. It is trained on wikipedia dataset and
embedded into several dimensions (e.g., 50, 100, 200, 300). 
% We did not use BoW strategy
% for Bi-LSTM,LSTM, and CNN because these model requires words along with their
% sequence which BoW cannot offer. We use 200D GloVe embedding with a maximum sequence length of 100 to tokenize each sentence. For the baselines (SVM, and Logit), following Uddin and Khomh~\cite{Uddin-OpinionValue-TSE2019,Uddin-OpinerReviewAlgo-ASE2017}, 
% we used BoW (unigrams) as features.
%and sentences were padded to
%100 words. The use of bag of words as features negates the underlying strength of
%the three models (CNN, LSTM, Bi-LSTM) because the information about word
%sequencing is absent in a bag of words representation. 


%\subsubsection{Architectures} 
%We choose four traditional deep learning models that are used ubiquitously for classification e.g. Deep Neural Network(DNN)\cite{Hinton-DNN-IEEESPM2012}, Convolutional Neural Network(CNN)\cite{Valueva-CNN-MCS2020}, Recurrent Neural Network(RNN) \cite{rnn-model}, Long Term-Short Memory(LSTM)\cite{Hochreiter-LSTM-NeuralComputation}, Bidirectional Long Term-Short Memory(BiLSTM) \cite{Huang-biLSTM-Arxiv2015}, and LSTM based Attention Model \cite{wang2016attention-based}. We investigate the performance of these models for sentiment classification task to get insight into models validity for our case. Dang at el.\cite{Dang_2020} and Ain at el.\cite{Ain2017} showed comparative analysis of different deep learning models e.g DNN, RNN, and CNN for sentiment analysis across different datasets. Alharbi at el.\cite{ALHARBI201950} applied CNN, and LSTM and Abid at el.\cite{ABID2019292} applied Bi-LSTM, and CNN model for twitter sentiment classification. Hameed et al.\cite{bilstm_hameed} reported that Single-Layered BiLSTM Model performed better than other deep models for sentiment detection in short sentences. Wang at el.\cite{wang-etal-2016-attention} used attention based LSTM model for aspect-label sentiment detection of customer review in a single sentence. A short description of these model are given below-\\ 
%\textbf{DNN}: This architecture first takes input of bags of words. This input layer is feed into a fully connected layer of size 128 followed by output layer of size 1. Sigmoid activation is used in output layer thus model predict a sentence as security related only if output is greater or equal to 0.5.\\
%\textbf{CNN}: CNN takes embedded sentences as input e.g. 100x200 dimension. These inputs are feed into a convolutional layers of 256 filters followed by a dropout layer, Max-Pooling layer, Flatten layer, then a fully connected layer of size 32 and finally an output layer with sigmoid activation. This architecture has a total of 400K trainable parameters.\\
\subsection{Transformer Models}\label{sec:background-transformer}
\nd\bf{\ul{Studied Models.}} Transformers are attention based deep models that can handle sequential data like RNN, LSTM. Unlike LSTM, these model can process unordered sequential data. This allows the models much more parallelism during the training and hence these models are faster than RNN, LSTM. Utilizing this feature, models are trained on large training dataset that was previously difficult using LSTM, RNN. These trained models are used for various language specific tasks e.g. aspect detection, sentiment detection, translation, etc  using downstream fine-tuning.  
We investigate five state-of-the-art transformer models: \begin{inparaenum}[(1)]
\item BERT~\cite{Delvin-BERTArch-Arxiv2018},
\item RoBERTa~\cite{Liu-Roberta-Arxiv2019}, 
\item XLNet~\cite{Yang-Xlnet-Arxiv2020}, 
\item DistillBERT~\cite{Sanh-DistillBERT-Arxiv2019}, 
\item Albert~\cite{Lan-Albert-Arxiv2020}, 
%\item ELECTRA~\cite{Clark-Electra-Arxiv2020}, and
%\item FunnelBERT~\cite{Dai-FunnelBERT-Arxiv2020}. 
\end{inparaenum}
% BERT is designed to learn pre-trained contextual word representation by running of large volume of 
% unlabeled texts. The bidirectional transfer encoder in BERT is multi-layer, which 
% offers robust contextual learning of word embeddings. As we find from RQ1, contextual learning 
% in Bi-LSTM contributed to its superior performance over CNN and DNN. Among the models we studied, 
% RoBERTa (Robustly Optimized BERT approach) is found to offer an upgrade on the BERT-base model due to 
% its modification of the pre-trained steps in BERT. We, therefore, pick RoBERTa over the BERT-base model in this study. 
% The second model in our study, XLNet is found to offer better performance on long texts by combining 
% the strengths of autoregressive (AR) and autoenconding (AE) language modeling and by integrating 
% the Transformer-XL. Albert is a lightweight version of BERT based on fewer number of parameters but with a larger architecture than BERT. 
% Albert is designed address to run with less computational resources than BERT, but is also found to outperform BERT-base 
% on a number of benchmark datsets (e.g., GLUE). ELECTRA trains two transformer models, a generator and a discriminator. The dual models 
% approach found to substantially outperform BERT-base given the same model size and data. FunnelBERT is similar to ELECTRA, but it intends to 
% reduce computational cost by gradually compressing the sequence of hidden states. 
%Edited

\begin{figure}
    \centering
    \includegraphics[scale=.65]{images/BERT_Archi_and_Clf.pdf}
    \caption{BERT Architecture Overview and Classification Processing}
    \label{fig:BERT}
\end{figure}
\nd\bf{\ul{Model Architecture.}} \fig\ref{fig:BERT} (left) shows the internal
architecture of Bidirectional Encoder Representations from Transformers (BERT)
model. BERT takes embedded representation $(E_i)$ of words and does some multi-headed
attention computation to create new intermediate representation $(Trm)$. Every
layer compute multi-headed attention on the previous intermediate representation
to create new one of identical size. The last intermediate layer of each word is
fed to create final contextualized representation($T_i$) for each word. {BERT} is trained on a large corpus like wikipedia, books, articles, and
etc in a self-supervised fashion to learn contextual word representation. This
means it was pretrained on the raw texts only, with no humans labelling them. It
is an automatic process to generate inputs and labels from those texts. These
models were pretrained with two objectives i) Masked Language
Modeling(MLM)\cite{salazar-etal-2020-masked} and ii) Next Sentence
Prediction(NSP)\cite{shi-demberg-2019-next-sentence-prediction}. BERT follow MLM
means model only predicts masked token instead of every next token. This is
because in multilayered model, lower layers leak information and allow a token
to itself in later layers. BERT model randomly masks 15\% of the words of a
sentence in the input then run the entire masked sentence through the model and
has to predict the masked words. It allows the model to learn a bidirectional
representation of the sentence. For NSP, model concatenates two masked sentences
as inputs during pretraining and then model predicts if the two sentences were
following each other or not. This way, model learns an inner representation of
the language that is used to extract features useful for downstream tasks.
Delvin at el.\cite{Delvin-BERTArch-Arxiv2018} provides two different
implementation of BERT e.g. BERT-Base and BERT-Large. BERT-Base has a parameters
of 110M with 12 layers, a hidden layer size of 768, and 12 self-attention heads.
In comparison, BERT-Large has 340M parameters with 24 layers, a hidden layer
size of 1,024, and 16 self-attention heads. Considering our dataset only
consists of 10K samples which are not enough to tune 340M parameters, we choose
BERT-Base model as suggested by Zhang at
el.\cite{Zhang-SentimentDetectionSEBERT-ICSME2020}. \fig\ref{fig:BERT} (right) 
shows how we used the BERT architecture for our security aspect detection.
At first, a tokenizer takes the input sentences and represents the tokenized
sentences. Then, this tokenized sentences are fed into BERT model. Finally, the
embedded sentences are passed through the classifier to get final
output (security or non-security).
%\gias{draw an explain a BERT architecture similar to \url{https://www.analyticsvidhya.com/blog/2019/09/demystifying-bert-groundbreaking-nlp-framework/}}
%\gias{use the above architecture to explain how BERT differs from LSTM and Bi-LSTM}

{XLNet} XLNet is pre-trained using an autoregressive method to learn bidirectional contexts by maximizing the expected likelihood over all permutations of the input sequence factorization order. Like BERT, this model also use the BooksCorpus and English Wikipedia as part of pretraining
data. In addition, Giga5, ClueWeb 2012-B, and Common Crawl data were used for pretraining. Yang at el.\cite{Yang-Xlnet-Arxiv2020} proposed this model showing under comparable experiment settings, XLNet outperforms BERT on 20 tasks, often by a large margin, including question answering, natural language inference, sentiment analysis, and document ranking. Similar to BERT, we choose XLNet-Base model.
{RoBERTa} RoBERTa is the most used and optimized BERT model for classification task. Roberta model is pretrained on BookCorpus, a dataset consisting of 11,038 unpublished books, English Wikipedia (excluding lists, tables and headers), CC-News: a dataset containing 63 millions English news articles, OpenWebText: an opensource recreation of the WebText,
Stories: a dataset containing a subset of CommonCrawl data. Contrary to BERT, the masking is done dynamically during pretraining (e.g., it changes at each epoch and is not fixed) \cite{Liu-Roberta-Arxiv2019}.
% Most used RoBERTa model is Roberta-Base. It has 125M parameters with 12 layers, 768 neurons per layer and 12 self-attention heads. 
{DistilBERT} DistilBERT is smaller and faster than BERT, which was pretrained on the same corpus, using the BERT base model as a teacher. This model has a triple loss combining language modeling, distillation and cosine-distance losses that makes the model smaller in parameter size while preserved in performance. Model has 40\% lesser parameters than its base model BERT. Following Pipalia at el.\cite{Distil-Bert} and Adoma at el.\cite{Adoma-Distil-Bert}, we use DistilBERT-Base model for our classification task.
% Model has 6 layers, a hidden layer size of 768, 12 self-attention heads and 66M parameters.
{ALBERT} This model also pretrained on similar dataset like BERT. It presents two parameter-reduction techniques, i)splitting the embedding matrix into two smaller matrices, and ii) using repeating layers split among groups, to lower memory consumption and increase the training speed. However, the computational cost remains similar to a BERT-like architecture with the same number of hidden layers as it has to iterate through the same number of (repeating) layers \cite{Lan-Albert-Arxiv2020}. There are two version of this model e.g. Albert-v1 and Albert-v2. These two models have different dropout rates, additional training data, and longer training. We use Albert-v2 for our experiments because it outperforms its previous version in downstream classification task.
% Model has 12 layers with 768 neurons per layers, 12 self-attentions and 11M parameters. 

%\textbf{FunnelBERT} FunnelBERT is pretrained on BookCorpus, a dataset consisting of 11,038 unpublished books, English Wikipedia (excluding lists, tables and headers), Clue Web: a dataset of 733,019,372 English web pages, GigaWord: an archive of newswire text data, and Common Crawl: a dataset of raw web pages. Model is similar like BERT except it uses pooling after each block of layers that makes the model more effective in downstream classification. The sequence length of the hidden states changes after each block of layers. The base model therefore has a final sequence length that is a quarter of the original one.
% Dai at el.\cite{Dai-FunnelBERT-Arxiv2020} proposed three different architectures e.g. FunnelBERT-Samll-Base, FunnelBERT-Medium-Base, and FunnelBERT-Large-Base of FunnelBERT. FunnelBERT-Samll-Base has the lowest 115M parameters with 12 layers, 768 neurons per hidden layer, and 12 self-attention heads among these three. We pick this model because other two have a huge parameters. 

%\textbf{ELECTRA} ELECTRA has nearly no changes to the underlying model, BERT except the separation of the embedding size and the hidden size. The embedding size is generally smaller, while the hidden size is larger. An additional linear projection layer is used to project the embeddings from their embedding size to the hidden size. Following the performance of this model for classification task shown by Clark at el.\cite{Clark-Electra-Arxiv2020}, we use this model for our experiment.
% Our used Electra-Small model has 12 layers, 256 neurons per hidden layer, 12 attention head and 14M parameters.

\begin{table}[t]
\centering
\caption{Architecture details of variants of BERT Model (L = Layers, H = Hidden, D = Heads, P = Parameters)}
\begin{tabular}{l|p{3.2cm}rrrr}
\toprule
\textbf{Architecture}& \bf{Used Model} & \bf{L}  & \bf{H} & \bf{D} & \bf{P}\\ 
\midrule
 BERT & bert-base-uncased & 12& 768&12&110M\\
 XLNet & xlnet-base-cased & 12& 768& 12& 110M                  \\ %\hline
 RoBERTa& roberta-base & 12&768&12&125M                               \\ %\hline
 DistilBERT &distilbert-base-uncased&  6& 768 & 12 & 66M                                \\
 ALBERT & albert-base-v1 & 12 &  768 & 12 & 11M \\
 %FunnelBERT & funnel-transformer/small-base &12& 768 & 12 & 115M \\
 %ELECTRA& google/electra-small-discriminator&  12&	256&12 &	14M\\
\bottomrule
\end{tabular}
%}
\label{architecture_details} 
%\end{center}
\end{table}
Table \ref{architecture_details} highlights the architectural details of the
used Transformer models in the the
\href{https://huggingface.co/transformers}{\textcolor{blue}{hugging face}}
transformer library, which is an open source community around the pre-trained
transformer libraries. BERT architecture provides the contextual embedding for
each word in a sentence. Now, for classification purpose, a classifier is used
at the top of the model which takes the embedding of sentences as input and
outputs the predicted weights for each category (Security and Non-Security). The
classifier consists of a fully connected layer, output layer, a softmax layer
and pooling layers with a total of around 2K trainable parameters. 
% For learning the weight of parameters, we use transfer learning \cite{Pan2010ASO} that means we initialize the weights from an already trained model and tune them for our classification task. We have already discuss the pretraining process of BERT model earlier this section. For tuning the parameters, we follow five steps- i) Model Initialization, ii) Sentence Tokenization, iii) Prediction, iv) Loss Calculation, and v) Parameter Tuning the, as shown in Figure \ref{fig:BERT-Training-Model}. We first initialize the parameters with pretrained weights found in hugging face. Then we tokenize and predict the class of the instance. We calculate the loss using cross entropy and back propagate the loss to update the parameters. 


% 
% \begin{figure}[t]
% %\vspace{-2mm}
% \centering
% %	\centering
%   	%\includegraphics[width=.49\textwidth,height=6cm]{images/opiner-resolver-true.png}
%   	\includegraphics[scale=.3]{images/BERT_Classifier.pdf}
%   	\caption{BERT Classification  Steps}
%   	 \label{fig:Bert Classifier}
% \vspace{-5mm}
% \end{figure}


\nd\bf{\ul{Model Features.}} We used the pre-trained embedding in BERT models, which learn 
additional contextual information for a given domain (e.g., in our case security in developer discussions) during 
the training phase. The combination of pre-trained and domain-specific learning into such pre-trained 
models offers those more contextual information during classification tasks than traditional DL models. 
 We added `EOS' and `CLS' to each sentence and then tokenized all sentences using pretrained BERT-Tokenizer. We
padded each sentences to 100 length with `zero' padding.

%\subsubsection{Architecture} 
% \begin{figure}
%     \centering
%     \includegraphics[scale=.15]{images/BERT.pdf}
%     \caption{BERT Architecture}
%     \label{fig:BERT Model}
% \end{figure}
% 
% \subsubsection{Architecture} 
% \begin{figure}
%     \centering
%     
%     \includegraphics[scale=.5]{images/Training.pdf}
%     \caption{BERT Training Process}
%     \label{fig:BERT-Training-Model}
% \end{figure}
% \begin{figure}[t]
% %\vspace{-2mm}
% \centering
% %	\centering
%   	%\includegraphics[width=.49\textwidth,height=6cm]{images/opiner-resolver-true.png}
%   	\includegraphics[scale=.75]{images/BERT.pdf}
%   	\caption{BERT Architecture}
%   	 \label{fig:Bert Architecture}
% \vspace{-5mm}
% \end{figure}

%\gias{if it helps, draw a diagram of the architecture}







%Edited

